Photodetection Aspects of JEM-EUSO and Studies of the Ultra-High Energy Cosmic Ray Sky

In this thesis, an introduction to the Ultra-High Energy Cosmic Ray (UHECR) field is given, including air shower physics, UHECR astrophysics, and experimental techniques. The current questions in UHECR physics are mentioned, along with the experimental challenges encountered in the field. The physics of air fluorescence is also presented, and the JEM-EUSO experiment is introduced in detail. The original contributions in this thesis are divided into experimental work on photodetection aspects of JEM-EUSO and phenomenological studies of UHECR composition and source statistics. A comprehensive introduction to photomultiplier tubes (PMTs) and single photoelectron counting are given, and the measurement of PMT efficiency with an uncertainty of a few percent is discussed in detail. An experimental setup for measuring the air fluorescence yield is also introduced, and tests of the EUSO-Balloon high voltage power supply prototype are presented. A setup for sorting the JEM-EUSO PMTs is developed, including the assembly and calibration of data acquisition hardware and the development of acquisition and analysis software. This system is used to perform an absolute calibration of the EUSO-Balloon focal surface, along with measurements of the PMT pixel width and dead-space. In the phenomenological part of this work, it is shown that a distribution of source maximum energies must be considered in order to understand the energy spectrum and the composition of UHECRs. The number of sources which can be expected to contribute to the UHECR sky is also studied, finding that on the order of 1 source(s) contributes more than 50% of the flux at 100 EeV.

==> IntroToCalibration.tex <==
\section{What is Calibration}

It would be beneficial at this point to consider what we actually mean when we speak of calibration. Calibration is, at its core, a complete understanding of the response of a measurement instrument or detector.
It is this understanding that allows us to make a true measurement or observation of an unknown phenomena. 

For a measurement device, such a meter-stick or a watch, this idea is clear. Imagine that I measure a length with wooden pole. The calibration of this ``instrument'' relative to a well defined unit, such as a meter, is uncertain at best.
If, afterward, I measure the pole itself with an actual meter-stick then my instrument is now a calibrated device. The question is then how well did I do in the calibration procedure and how accurate was the meter-stick which I used. 
If I compared the pole to the meter-stick only very hastily or the marks on the meter-stick where worn off, it may well be that my calibration was mediocre at best. I could improve these two points, and therefore the accuracy of every measurement which
I make with my device, by developing a well-thought out procedure for the comparison and by comparing my device to a universal and repeatable length, such a the distance lights travels in a given unit of time.

It can already be seen that the act of calibration is fundamental to any precise measurement. 

The method of calibration falls into two broad areas: Calibration against a known source or phenomena and calibration against another known device.  


==> tables/AirFluorescencePMTCalibration/VoltageRepartitions.tex <==
% \begin{table} 
%  \begin{center}
% \begin{tabulary}{1.2\textwidth}{LCCCCCCCCCCCCCCC}
% 
% \toprule
% ~ & \small K & \small G & \small D1 & \small D2 & \small D3 & \small D4 & \small D5 & \small D6 & \small D7 & \small D8 & \small D9 & \small D10 & \small D11 & \small D12  & \small Total\\
% \cmidrule(l){2-16}
% \small Type A  & \small1.2 & \small 2.8 & \small 1.2 & \small 1.8 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1  & \small 17 \\
% \small Type C  & \small1.2 & \small 2.8 & \small 1.2 & \small 1.8 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1 & \small 1.5 & \small 1.5 & \small 3 & \small 2.5 & \small 21.5 \\
% \bottomrule
% \end{tabulary}
% \caption[XP2020Q Voltage Repartition]{
% \label{tab:XP2020QvoltageRepartions}
% (Maximum Gain) (linearity)
% }
%  \end{center}
% \end{table}

\begin{table}
 \begin{center}
\begin{tabulary}{1.0\textwidth}{LCC}

\toprule
Element & \multicolumn{2}{c}{Type}\\
 \cmidrule(l){2-3}
 &  A & C\\
\cmidrule(l){1-3}
K & 1.2 & 1.2 \\
G & 2.8 & 2.8 \\
D1 & 1.2 & 1.2 \\
D2 & 1.8 & 1.8 \\
D3 & 1 & 1 \\
D4 & 1 & 1 \\
D5 & 1 & 1 \\
D6 & 1 & 1 \\
D7 & 1 & 1 \\
D8 & 1 & 1 \\
D9 & 1 & 1.5 \\
D10 & 1 & 1.5 \\
D11 & 1 & 3 \\
D12 & 1 & 2.5 \\
Total & 17 & 21.5 \\
\bottomrule
\end{tabulary}
\caption[XP2020Q Voltage Repartition]{
\label{tab:XP2020QvoltageRepartions}
Table showing the Type A and Type C voltage repartitions recommended by Photonis for the XP2020Q. The Type C distribution is recommended for good linearity, while the Type A is recommended for maximum gain. 
For each powered element of the PMT the voltage step between it and the next element is given as a fraction the step voltage which is the supply voltage divided by the total number of steps. For example, 
the at a supply voltage of 2000 V the voltage step in the C distribution is $93 \frac{1}{43}$ and the voltage difference between the photocathode (K) and the focusing element (G) should be $111 \frac{27}{43}$. 
}
 \end{center}
\end{table}

==> tables/C205CalibrationsReport/C205_n69_table.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{r|c}
Channel & Conversion Constant  \\ 
 & [ fC / count ] $\pm~0.24~ \%$  \\	\hline	
$ 1 $&$ 28.88 $\\
$ 2 $&$ 28.69 $\\
$ 3 $&$ 29.00 $\\
$ 4 $&$ 28.92 $\\
$ 5 $&$ 29.03 $\\
$ 6 $&$ 29.19 $\\
$ 7 $&$ 29.09 $\\
$ 8 $&$ 29.15 $\\
$ 9 $&$ 28.99 $\\
$ 10 $&$ 28.89 $\\
$ 11 $&$ 28.91 $\\
$ 12 $&$ 29.00 $\\
$ 13 $&$ 28.84 $\\
$ 14 $&$ 28.79 $\\
$ 15 $&$ 28.68 $\\
$ 16 $&$ 28.93 $\\
$ 17 $&$ 29.16 $\\
$ 18 $&$ 29.08 $\\
$ 19 $&$ 29.20 $\\
$ 20 $&$ 29.18 $\\
$ 21 $&$ 29.06 $\\
$ 22 $&$ 29.06 $\\
$ 23 $&$ 29.14 $\\
$ 24 $&$ 29.01 $\\
$ 25 $&$ 29.17 $\\
$ 26 $&$ 29.16 $\\
$ 27 $&$ 29.08 $\\
$ 28 $&$ 29.08 $\\
$ 29 $&$ 29.03 $\\
$ 30 $&$ 29.25 $\\
$ 31 $&$ 28.95 $\\
$ 32 $&$ 29.18 $\\
\end{tabular}
\caption[C205 n69 Conversion Constants]{Conversion Constants measured for each channel of C205, module number 69. The total relative error for all channels is $\pm~0.24~ \%$.
This error is  calculated idependently for each channel and rounded up to 2 significant figures.}
\label{tab:C205n69CC}
\end{center}
\end{table}

==> tables/C205CalibrationsReport/C205_n75_table.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{r|c}
Channel & Conversion Constant  \\ 
 & [ fC / count ] $\pm~0.25~ \%$ \\ \hline	
$ 1 $&$ 29.12 $\\
$ 2 $&$ 29.20 $\\
$ 3 $&$ 29.02 $\\
$ 4 $&$ 28.91 $\\
$ 5 $&$ 29.08 $\\
$ 6 $&$ 28.98 $\\
$ 7 $&$ 29.07 $\\
$ 8 $&$ 29.09 $\\
$ 9 $&$ 28.86 $\\
$ 10 $&$ 28.98 $\\
$ 11 $&$ 28.9 $\\
$ 12 $&$ 29.02 $\\
$ 13 $&$ 28.78 $\\
$ 14 $&$ 29.04 $\\
$ 15 $&$ 28.79 $\\
$ 16 $&$ 29.00 $\\
$ 17 $&$ 28.89 $\\
$ 18 $&$ 28.96 $\\
$ 19 $&$ 29.17 $\\
$ 20 $&$ 28.92 $\\
$ 21 $&$ 28.87 $\\
$ 22 $&$ 28.82 $\\
$ 23 $&$ 29.36 $\\
$ 24 $&$ 28.88 $\\
$ 25 $&$ 28.95 $\\
$ 26 $&$ 29.35 $\\
$ 27 $&$ 29.07 $\\
$ 28 $&$ 29.20 $\\
$ 29 $&$ 29.23 $\\
$ 30 $&$ 29.23 $\\
$ 31 $&$ 29.13 $\\
$ 32 $&$ 29.08 $\\ 
\end{tabular}
\caption[C205 n75 Conversion Constants]{Conversion Constants measured for each channel of C205, module number 75. The total relative error for all channels is $\pm~0.25~ \%$.
This error is calculated idependently for each channel and rounded up to 2 significant figures. }
\label{tab:C205n69CC}
\end{center}
\end{table}

==> tables/CalibrationSetup/ISphereSurfaceAreas.tex <==
\begin{table}
 \begin{center}
 \begin{tabulary}{1.25\textwidth}{LCC}
 
\toprule 
Element & diameter & Surface Area \\
\cmidrule(r){1-3}
$A_{\text{sphere}}$ (Total Sphere) & 10.16 cm (4 in) & $324.3~cm^{2}$\\
$A_{\text{port 1}}$ & 3.81 cm (1.5 in) & $11.4~cm^{2}$\\
$A_{\text{port 2}}$ & 2.54 cm (1.0 in) & $5.0~cm^{2}$\\
$A_{\text{port 1}}$ & 2.54 cm (1.0 in) & $5.0~cm^{2}$\\
$A_{\text{eff}}$ (Effective) & -- & $81~cm^{2}$\\
$A_{\text{NIST}}$ (photodiode) & 9 mm  & $81~cm^{2}$\\
\bottomrule
\end{tabulary}
 \caption[Table of Integrating Sphere Areas]{
 A list of Integrating sphere dimensions and calculated surface areas, as a reference.
 }
 \end{center}
\end{table}

==> tables/EUSOBalloon-ECmeasurements/EC109_PMTA_AbsoluteMap_RefPixel051.tex <==
01 0.252 0.020 0.028 1.715
02 0.266 0.024 0.030 2.286
03 0.261 0.021 0.029 2.325
04 0.241 0.017 0.026 2.338
05 0.253 0.022 0.029 2.032
06 0.261 0.020 0.027 1.461
07 0.247 0.018 0.026 1.931
08 0.000 0.000 0.000 1.466
09 0.000 0.000 0.000 0.000
10 0.222 0.017 0.025 2.767
11 0.229 0.018 0.026 2.886
12 0.228 0.016 0.025 3.009
13 0.229 0.017 0.026 2.489
14 0.228 0.016 0.025 2.859
15 0.231 0.017 0.026 2.662
16 0.229 0.028 0.034 1.643
17 0.252 0.017 0.025 2.602
18 0.228 0.016 0.025 2.652
19 0.228 0.016 0.025 2.603
20 0.238 0.025 0.031 1.639
21 0.239 0.018 0.026 2.479
22 0.229 0.017 0.025 2.601
23 0.256 0.027 0.033 1.136
24 0.240 0.024 0.031 1.607
25 0.245 0.017 0.026 2.393
26 0.242 0.018 0.026 2.424
27 0.229 0.017 0.025 2.912
28 0.228 0.018 0.027 2.111
29 0.238 0.021 0.028 2.067
30 0.244 0.017 0.025 2.380
31 0.241 0.018 0.026 2.403
32 0.245 0.024 0.031 1.630
33 0.000 0.000 0.000 0.006
34 0.229 0.017 0.025 2.732
35 0.231 0.018 0.026 2.427
36 0.227 0.017 0.026 2.642
37 0.230 0.017 0.026 2.552
38 0.240 0.018 0.026 2.638
39 0.247 0.017 0.026 2.170
40 0.236 0.020 0.027 1.544
41 0.255 0.019 0.027 2.280
42 0.234 0.018 0.026 2.235
43 0.238 0.018 0.026 2.429
44 0.242 0.022 0.029 2.435
45 0.000 0.000 0.000 1.288
46 0.245 0.020 0.028 2.455
47 0.242 0.021 0.028 2.150
48 0.246 0.025 0.031 1.575
49 0.000 0.000 0.000 1.496
50 0.239 0.020 0.028 2.146
51 0.241 0.009 0.021 2.255
52 0.245 0.017 0.025 2.464
53 0.251 0.020 0.027 2.211
54 0.254 0.016 0.025 2.559
55 0.241 0.016 0.025 2.480
56 0.241 0.022 0.029 1.551
57 0.000 0.000 0.000 0.463
58 0.000 0.000 0.000 0.982
59 0.276 0.028 0.034 1.512
60 0.266 0.024 0.031 1.835
61 0.251 0.017 0.026 2.187
62 0.257 0.020 0.028 1.932
63 0.250 0.024 0.030 1.703
64 0.000 0.000 0.000 1.002


==> tables/EUSOBalloon-ECmeasurements/EC109_PMTB_AbsoluteMap_RefPixel022.tex <==
01 0.276 0.016 0.025 2.737
02 0.272 0.016 0.025 3.566
03 0.274 0.016 0.025 3.639
04 0.286 0.018 0.026 2.523
05 0.251 0.016 0.025 3.020
06 0.280 0.017 0.026 2.503
07 0.271 0.019 0.027 2.161
08 0.000 0.000 0.000 1.128
09 0.267 0.016 0.025 3.287
10 0.245 0.016 0.025 4.296
11 0.246 0.016 0.025 4.204
12 0.250 0.016 0.025 3.782
13 0.248 0.016 0.025 3.351
14 0.249 0.016 0.025 2.919
15 0.254 0.021 0.028 2.652
16 0.247 0.018 0.026 1.710
17 0.272 0.016 0.025 3.130
18 0.244 0.016 0.025 3.182
19 0.247 0.016 0.025 3.436
20 0.235 0.016 0.025 3.730
21 0.239 0.016 0.025 3.444
22 0.227 0.009 0.021 3.819
23 0.241 0.016 0.025 2.621
24 0.000 0.000 0.000 1.092
25 0.263 0.016 0.025 3.067
26 0.232 0.016 0.025 3.354
27 0.225 0.016 0.025 3.027
28 0.247 0.025 0.032 1.834
29 0.237 0.017 0.026 2.540
30 0.238 0.018 0.026 3.157
31 0.237 0.016 0.025 2.706
32 0.241 0.016 0.025 2.539
33 0.248 0.016 0.025 2.921
34 0.249 0.022 0.029 1.571
35 0.240 0.016 0.025 2.934
36 0.229 0.016 0.025 2.781
37 0.233 0.018 0.026 2.137
38 0.238 0.016 0.025 2.766
39 0.232 0.016 0.025 3.093
40 0.245 0.018 0.026 2.434
41 0.264 0.016 0.025 2.730
42 0.240 0.019 0.027 2.511
43 0.230 0.017 0.025 3.330
44 0.239 0.018 0.026 2.504
45 0.224 0.017 0.026 2.380
46 0.237 0.017 0.025 2.724
47 0.241 0.017 0.026 2.839
48 0.228 0.018 0.026 2.000
49 0.268 0.017 0.025 3.057
50 0.232 0.017 0.026 2.898
51 0.237 0.022 0.029 2.199
52 0.236 0.021 0.028 2.376
53 0.227 0.018 0.026 2.500
54 0.229 0.016 0.025 3.039
55 0.245 0.017 0.025 2.696
56 0.244 0.021 0.028 1.976
57 0.297 0.021 0.028 1.721
58 0.273 0.022 0.029 2.099
59 0.288 0.024 0.030 1.773
60 0.274 0.021 0.028 2.063
61 0.267 0.018 0.027 2.056
62 0.290 0.024 0.030 1.878
63 0.298 0.027 0.033 1.972
64 0.000 0.000 0.000 0.000


==> tables/EUSOBalloon-ECmeasurements/EC109_PMTC_AbsoluteMap_RefPixel022.tex <==
01 0.000 0.000 0.000 1.209
02 0.385 0.028 0.034 1.724
03 0.359 0.023 0.030 1.875
04 0.332 0.018 0.026 1.986
05 0.360 0.023 0.030 1.835
06 0.349 0.019 0.027 1.576
07 0.330 0.017 0.026 2.128
08 0.000 0.000 0.000 1.129
09 0.000 0.000 0.000 0.000
10 0.293 0.015 0.025 3.053
11 0.295 0.016 0.025 3.168
12 0.285 0.016 0.025 2.777
13 0.286 0.016 0.025 3.129
14 0.296 0.016 0.025 2.872
15 0.299 0.017 0.025 3.066
16 0.334 0.021 0.028 2.418
17 0.325 0.016 0.025 2.443
18 0.296 0.016 0.025 2.705
19 0.291 0.016 0.025 2.732
20 0.292 0.019 0.027 1.796
21 0.290 0.017 0.025 2.709
22 0.285 0.008 0.021 3.508
23 0.280 0.019 0.027 1.832
24 0.312 0.016 0.025 2.504
25 0.303 0.016 0.025 2.473
26 0.000 0.000 0.000 0.917
27 0.284 0.017 0.026 2.643
28 0.278 0.017 0.026 2.346
29 0.277 0.017 0.026 2.280
30 0.293 0.016 0.025 2.329
31 0.287 0.016 0.025 2.457
32 0.315 0.017 0.025 2.486
33 0.336 0.029 0.035 1.445
34 0.293 0.020 0.027 2.261
35 0.276 0.021 0.028 1.739
36 0.283 0.016 0.025 2.394
37 0.280 0.017 0.025 2.491
38 0.288 0.016 0.025 2.357
39 0.285 0.017 0.026 2.740
40 0.313 0.016 0.025 2.228
41 0.296 0.019 0.027 2.068
42 0.275 0.018 0.026 1.828
43 0.282 0.020 0.027 2.151
44 0.278 0.017 0.025 2.083
45 0.288 0.024 0.031 1.950
46 0.281 0.016 0.025 2.626
47 0.289 0.016 0.025 2.399
48 0.313 0.016 0.025 2.430
49 0.000 0.000 0.000 0.964
50 0.273 0.020 0.028 1.379
51 0.297 0.022 0.029 1.569
52 0.286 0.015 0.025 2.653
53 0.273 0.020 0.028 2.091
54 0.290 0.015 0.024 3.074
55 0.291 0.016 0.025 2.763
56 0.311 0.016 0.025 2.402
57 0.000 0.000 0.000 0.516
58 0.000 0.000 0.000 0.618
59 0.000 0.000 0.000 1.175
60 0.324 0.021 0.028 1.374
61 0.327 0.016 0.025 2.472
62 0.320 0.016 0.025 2.534
63 0.314 0.017 0.026 2.441
64 0.330 0.022 0.029 1.701


==> tables/EUSOBalloon-ECmeasurements/EC109_PMTD_AbsoluteMap_RefPixel051.tex <==
01 0.300 0.020 0.028 1.865
02 0.296 0.016 0.025 2.614
03 0.295 0.017 0.025 2.735
04 0.293 0.019 0.027 2.200
05 0.287 0.016 0.025 2.578
06 0.328 0.030 0.035 1.475
07 0.314 0.024 0.031 1.798
08 0.000 0.000 0.000 0.794
09 0.296 0.016 0.025 3.271
10 0.281 0.015 0.024 3.683
11 0.283 0.015 0.024 3.562
12 0.278 0.015 0.024 3.637
13 0.262 0.015 0.025 3.330
14 0.257 0.015 0.024 2.939
15 0.269 0.016 0.025 1.894
16 0.000 0.000 0.000 1.202
17 0.296 0.015 0.024 3.118
18 0.273 0.015 0.024 3.831
19 0.272 0.015 0.024 4.169
20 0.271 0.015 0.024 3.510
21 0.266 0.015 0.024 3.504
22 0.264 0.016 0.025 3.304
23 0.277 0.016 0.025 2.982
24 0.000 0.000 0.000 1.338
25 0.295 0.015 0.024 2.952
26 0.278 0.015 0.025 2.841
27 0.269 0.015 0.024 3.267
28 0.280 0.020 0.028 2.369
29 0.271 0.016 0.025 2.924
30 0.266 0.016 0.025 2.672
31 0.264 0.015 0.024 3.063
32 0.314 0.018 0.026 2.527
33 0.299 0.015 0.024 2.501
34 0.295 0.021 0.028 2.299
35 0.269 0.015 0.025 3.269
36 0.262 0.015 0.024 3.204
37 0.276 0.019 0.027 2.167
38 0.269 0.015 0.024 3.057
39 0.270 0.015 0.024 3.111
40 0.293 0.016 0.025 2.537
41 0.298 0.015 0.025 2.942
42 0.263 0.015 0.025 3.191
43 0.269 0.015 0.025 3.453
44 0.274 0.016 0.025 2.789
45 0.263 0.016 0.025 3.185
46 0.261 0.015 0.024 3.494
47 0.276 0.015 0.024 3.273
48 0.301 0.016 0.025 2.454
49 0.316 0.021 0.028 2.156
50 0.285 0.016 0.025 2.948
51 0.277 0.008 0.021 2.783
52 0.262 0.015 0.024 3.340
53 0.272 0.016 0.025 3.072
54 0.269 0.015 0.024 3.152
55 0.286 0.015 0.024 3.201
56 0.292 0.017 0.025 2.340
57 0.000 0.000 0.000 0.827
58 0.000 0.000 0.000 1.018
59 0.319 0.022 0.029 1.530
60 0.315 0.019 0.027 1.825
61 0.308 0.019 0.027 2.087
62 0.296 0.017 0.025 1.854
63 0.307 0.017 0.026 2.314
64 0.000 0.000 0.000 0.000


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC101_PMTA_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC101--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.327 & 33 & -- & -- &0.615 \\
02 & -- & -- &0.851 & 34 & -- & -- &0.275 \\
03 & -- & -- &0.896 & 35 & -- & -- &0.536 \\
04 & -- & -- &0.855 & 36 & -- & -- &0.842 \\
05 & -- & -- &0.855 & 37 & -- & -- &0.357 \\
06 & -- & -- &0.686 & 38 & -- & -- &1.309 \\
07 & -- & -- &0.455 & 39 & -- & -- &0.686 \\
08 & -- & -- &0.308 & 40 & -- & -- &1.345 \\
09 & -- & -- &0.360 & 41 & -- & -- &0.624 \\
10 & -- & -- &0.813 & 42 & -- & -- &1.055 \\
11 & -- & -- &0.858 & 43 & -- & -- &0.450 \\
12 & -- & -- &0.748 & 44 & -- & -- &3.246 \\
13 & -- & -- &0.485 & 45 & -- & -- &0.056 \\
14 & -- & -- &0.436 & 46 & -- & -- &14.819 \\
15 & -- & -- &0.292 & 47 & -- & -- &0.978 \\
16 & -- & -- &1.004 & 48 & -- & -- &0.845 \\
17 & 0.289 & 0.025 & 1.275 & 49 & -- & -- &0.571 \\
18 & -- & -- &0.761 & 50 & -- & -- &0.737 \\
19 & -- & -- &0.840 & 51 & -- & -- &0.402 \\
20 & -- & -- &19.391 & 52 & -- & -- &1.020 \\
21 & -- & -- &0.854 & 53 & -- & -- &0.803 \\
22 & -- & -- &0.263 & 54 & 0.250 & 0.037 & 1.338 \\
23 & -- & -- &0.924 & 55 & 0.234 & 0.036 & 1.196 \\
24 & -- & -- &0.864 & 56 & -- & -- &0.962 \\
25 & -- & -- &1.196 & 57 & -- & -- &0.618 \\
26 & -- & -- &1.212 & 58 & -- & -- &0.637 \\
27 & -- & -- &1.075 & 59 & -- & -- &0.406 \\
28 & -- & -- &0.801 & 60 & -- & -- &0.234 \\
29 & -- & -- &0.796 & 61 & -- & -- &1.106 \\
30 & -- & -- &0.976 & 62 & -- & -- &0.929 \\
31 & -- & -- &0.837 & 63 & -- & -- &1.037 \\
32 & -- & -- &0.764 & 64 & -- & -- &0.394 \\
\bottomrule
\end{tabulary}
\caption[EC101--PMTA Efficiency Results]{ \label{tab:EC101--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC101_PMTB_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC101--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.266 & 33 & 0.267 & 0.035 & 1.446 \\
02 & -- & -- &1.393 & 34 & 0.242 & 0.034 & 1.450 \\
03 & -- & -- &1.466 & 35 & -- & -- &1.333 \\
04 & -- & -- &0.901 & 36 & -- & -- &1.007 \\
05 & -- & -- &1.122 & 37 & -- & -- &0.528 \\
06 & -- & -- &0.454 & 38 & -- & -- &1.080 \\
07 & -- & -- &0.830 & 39 & -- & -- &0.948 \\
08 & -- & -- &0.551 & 40 & -- & -- &1.277 \\
09 & 0.250 & 0.033 & 1.303 & 41 & 0.272 & 0.035 & 1.549 \\
10 & 0.233 & 0.027 & 2.008 & 42 & -- & -- &1.287 \\
11 & 0.243 & 0.030 & 2.091 & 43 & -- & -- &1.175 \\
12 & 0.235 & 0.029 & 1.785 & 44 & -- & -- &1.169 \\
13 & -- & -- &1.246 & 45 & -- & -- &1.287 \\
14 & -- & -- &0.853 & 46 & -- & -- &1.218 \\
15 & -- & -- &1.134 & 47 & 0.255 & 0.036 & 1.384 \\
16 & -- & -- &1.264 & 48 & -- & -- &1.003 \\
17 & 0.269 & 0.034 & 1.623 & 49 & -- & -- &1.092 \\
18 & 0.247 & 0.034 & 1.401 & 50 & -- & -- &0.741 \\
19 & 0.235 & 0.031 & 1.734 & 51 & -- & -- &0.546 \\
20 & -- & -- &1.267 & 52 & -- & -- &0.350 \\
21 & 0.247 & 0.031 & 1.550 & 53 & -- & -- &0.399 \\
22 & 0.270 & 0.023 & 1.624 & 54 & -- & -- &0.589 \\
23 & -- & -- &1.244 & 55 & -- & -- &0.878 \\
24 & -- & -- &0.361 & 56 & -- & -- &1.197 \\
25 & 0.269 & 0.035 & 1.716 & 57 & -- & -- &0.746 \\
26 & 0.235 & 0.032 & 1.741 & 58 & -- & -- &0.186 \\
27 & -- & -- &1.326 & 59 & -- & -- &0.402 \\
28 & -- & -- &0.753 & 60 & -- & -- &0.059 \\
29 & -- & -- &0.887 & 61 & -- & -- &0.706 \\
30 & -- & -- &1.318 & 62 & -- & -- &0.170 \\
31 & -- & -- &1.215 & 63 & -- & -- &0.486 \\
32 & -- & -- &0.943 & 64 & -- & -- &0.874 \\
\bottomrule
\end{tabulary}
\caption[EC101--PMTB Efficiency Results]{ \label{tab:EC101--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC101_PMTC_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC101--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.365 & 33 & -- & -- &0.538 \\
02 & -- & -- &0.563 & 34 & -- & -- &1.032 \\
03 & -- & -- &0.641 & 35 & -- & -- &1.010 \\
04 & -- & -- &1.045 & 36 & -- & -- &1.475 \\
05 & -- & -- &0.334 & 37 & -- & -- &1.165 \\
06 & -- & -- &0.577 & 38 & 0.293 & 0.035 & 1.415 \\
07 & -- & -- &0.604 & 39 & 0.278 & 0.034 & 1.475 \\
08 & -- & -- &0.312 & 40 & 0.284 & 0.030 & 1.772 \\
09 & -- & -- &0.760 & 41 & -- & -- &0.818 \\
10 & -- & -- &1.312 & 42 & -- & -- &1.001 \\
11 & -- & -- &1.215 & 43 & 0.266 & 0.032 & 1.565 \\
12 & -- & -- &0.998 & 44 & -- & -- &1.249 \\
13 & -- & -- &0.942 & 45 & -- & -- &0.964 \\
14 & -- & -- &1.362 & 46 & 0.274 & 0.036 & 1.438 \\
15 & -- & -- &1.216 & 47 & 0.256 & 0.028 & 1.885 \\
16 & -- & -- &1.235 & 48 & 0.271 & 0.028 & 1.944 \\
17 & -- & -- &1.388 & 49 & -- & -- &0.678 \\
18 & -- & -- &1.174 & 50 & -- & -- &0.920 \\
19 & 0.291 & 0.037 & 1.349 & 51 & -- & -- &0.807 \\
20 & -- & -- &0.743 & 52 & 0.245 & 0.028 & 1.861 \\
21 & -- & -- &1.417 & 53 & -- & -- &0.913 \\
22 & 0.283 & 0.022 & 1.660 & 54 & 0.271 & 0.033 & 2.273 \\
23 & 0.278 & 0.032 & 1.697 & 55 & 0.253 & 0.028 & 2.373 \\
24 & 0.302 & 0.031 & 1.839 & 56 & 0.259 & 0.028 & 2.081 \\
25 & -- & -- &1.318 & 57 & -- & -- &0.359 \\
26 & 0.278 & 0.034 & 1.590 & 58 & -- & -- &0.393 \\
27 & 0.257 & 0.028 & 1.473 & 59 & -- & -- &0.301 \\
28 & 0.284 & 0.033 & 1.335 & 60 & -- & -- &1.017 \\
29 & -- & -- &1.251 & 61 & 0.312 & 0.036 & 1.225 \\
30 & 0.286 & 0.032 & 1.600 & 62 & -- & -- &1.123 \\
31 & 0.284 & 0.034 & 1.602 & 63 & 0.296 & 0.032 & 1.567 \\
32 & -- & -- &1.464 & 64 & -- & -- &0.696 \\
\bottomrule
\end{tabulary}
\caption[EC101--PMTC Efficiency Results]{ \label{tab:EC101--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC101_PMTD_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC101--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.249 & 0.032 & 1.572 & 33 & 0.257 & 0.033 & 1.413 \\
02 & 0.260 & 0.033 & 1.472 & 34 & -- & -- &1.239 \\
03 & -- & -- &1.427 & 35 & -- & -- &1.108 \\
04 & -- & -- &0.441 & 36 & -- & -- &0.798 \\
05 & -- & -- &1.174 & 37 & -- & -- &0.248 \\
06 & -- & -- &0.737 & 38 & -- & -- &0.866 \\
07 & -- & -- &0.929 & 39 & -- & -- &0.811 \\
08 & -- & -- &0.380 & 40 & -- & -- &1.006 \\
09 & 0.228 & 0.027 & 2.094 & 41 & -- & -- &1.167 \\
10 & 0.220 & 0.028 & 1.915 & 42 & -- & -- &1.106 \\
11 & 0.226 & 0.031 & 1.954 & 43 & -- & -- &1.204 \\
12 & 0.224 & 0.030 & 1.836 & 44 & -- & -- &0.902 \\
13 & -- & -- &0.979 & 45 & -- & -- &0.975 \\
14 & -- & -- &1.222 & 46 & -- & -- &1.068 \\
15 & -- & -- &0.607 & 47 & -- & -- &1.216 \\
16 & -- & -- &0.822 & 48 & -- & -- &0.813 \\
17 & 0.245 & 0.021 & 2.118 & 49 & -- & -- &0.694 \\
18 & 0.230 & 0.035 & 1.295 & 50 & -- & -- &0.385 \\
19 & 0.212 & 0.029 & 1.729 & 51 & -- & -- &0.388 \\
20 & -- & -- &1.086 & 52 & -- & -- &0.283 \\
21 & -- & -- &1.181 & 53 & -- & -- &0.641 \\
22 & -- & -- &0.891 & 54 & -- & -- &5.355 \\
23 & -- & -- &0.807 & 55 & -- & -- &0.481 \\
24 & -- & -- &0.306 & 56 & -- & -- &0.709 \\
25 & 0.238 & 0.028 & 2.012 & 57 & -- & -- &0.184 \\
26 & 0.218 & 0.031 & 1.655 & 58 & -- & -- &0.051 \\
27 & 0.228 & 0.035 & 1.260 & 59 & -- & -- &0.458 \\
28 & -- & -- &0.346 & 60 & -- & -- &0.120 \\
29 & -- & -- &0.359 & 61 & -- & -- &0.090 \\
30 & -- & -- &0.892 & 62 & -- & -- &0.875 \\
31 & -- & -- &0.634 & 63 & -- & -- &0.302 \\
32 & -- & -- &0.268 & 64 & -- & -- &0.578 \\
\bottomrule
\end{tabulary}
\caption[EC101--PMTD Efficiency Results]{ \label{tab:EC101--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC102_PMTA_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC102--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.327 & 33 & -- & -- &0.787 \\
02 & -- & -- &0.329 & 34 & -- & -- &1.147 \\
03 & -- & -- &0.591 & 35 & -- & -- &0.826 \\
04 & -- & -- &0.394 & 36 & -- & -- &0.903 \\
05 & -- & -- &0.837 & 37 & -- & -- &0.736 \\
06 & -- & -- &0.974 & 38 & -- & -- &1.000 \\
07 & -- & -- &0.887 & 39 & -- & -- &0.970 \\
08 & -- & -- &0.918 & 40 & -- & -- &1.097 \\
09 & -- & -- &0.565 & 41 & -- & -- &1.282 \\
10 & -- & -- &0.789 & 42 & 0.223 & 0.029 & 1.948 \\
11 & -- & -- &0.487 & 43 & -- & -- &1.076 \\
12 & -- & -- &0.329 & 44 & -- & -- &1.106 \\
13 & -- & -- &0.248 & 45 & -- & -- &0.971 \\
14 & -- & -- &0.130 & 46 & -- & -- &1.143 \\
15 & -- & -- &0.251 & 47 & -- & -- &1.102 \\
16 & -- & -- &0.903 & 48 & 0.288 & 0.037 & 1.368 \\
17 & 0.277 & 0.023 & 1.382 & 49 & 0.271 & 0.031 & 1.711 \\
18 & -- & -- &1.379 & 50 & 0.271 & 0.037 & 1.422 \\
19 & -- & -- &0.725 & 51 & -- & -- &0.731 \\
20 & -- & -- &0.312 & 52 & -- & -- &1.100 \\
21 & -- & -- &0.875 & 53 & -- & -- &0.592 \\
22 & -- & -- &0.984 & 54 & -- & -- &1.276 \\
23 & -- & -- &0.043 & 55 & -- & -- &1.081 \\
24 & -- & -- &1.064 & 56 & 0.292 & 0.037 & 1.386 \\
25 & -- & -- &1.065 & 57 & -- & -- &0.893 \\
26 & -- & -- &1.317 & 58 & -- & -- &1.365 \\
27 & -- & -- &1.121 & 59 & -- & -- &0.996 \\
28 & -- & -- &1.008 & 60 & -- & -- &0.778 \\
29 & -- & -- &0.793 & 61 & -- & -- &0.950 \\
30 & -- & -- &1.302 & 62 & -- & -- &0.186 \\
31 & -- & -- &1.153 & 63 & -- & -- &1.087 \\
32 & -- & -- &1.124 & 64 & -- & -- &0.357 \\
\bottomrule
\end{tabulary}
\caption[EC102--PMTA Efficiency Results]{ \label{tab:EC102--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC102_PMTB_AbsoluteMap_RefPixel033 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC102--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.216 & 33 & -- & -- &0.836 \\
02 & -- & -- &1.191 & 34 & -- & -- &1.031 \\
03 & -- & -- &1.075 & 35 & -- & -- &0.961 \\
04 & -- & -- &0.139 & 36 & -- & -- &1.831 \\
05 & -- & -- &0.949 & 37 & -- & -- &0.519 \\
06 & -- & -- &0.998 & 38 & -- & -- &0.594 \\
07 & -- & -- &1.319 & 39 & -- & -- &0.857 \\
08 & -- & -- &1.068 & 40 & -- & -- &1.138 \\
09 & -- & -- &1.219 & 41 & -- & -- &1.147 \\
10 & -- & -- &1.378 & 42 & -- & -- &1.031 \\
11 & -- & -- &1.493 & 43 & -- & -- &1.016 \\
12 & -- & -- &1.479 & 44 & -- & -- &0.401 \\
13 & -- & -- &1.270 & 45 & -- & -- &0.550 \\
14 & -- & -- &1.460 & 46 & -- & -- &0.935 \\
15 & -- & -- &1.405 & 47 & -- & -- &1.167 \\
16 & -- & -- &0.730 & 48 & -- & -- &1.230 \\
17 & -- & -- &1.348 & 49 & -- & -- &0.854 \\
18 & -- & -- &1.003 & 50 & -- & -- &0.651 \\
19 & -- & -- &1.325 & 51 & -- & -- &0.707 \\
20 & -- & -- &1.230 & 52 & -- & -- &49.908 \\
21 & -- & -- &1.164 & 53 & -- & -- &0.648 \\
22 & -- & -- &1.038 & 54 & -- & -- &0.396 \\
23 & -- & -- &1.157 & 55 & -- & -- &0.863 \\
24 & -- & -- &0.759 & 56 & -- & -- &0.791 \\
25 & -- & -- &1.650 & 57 & -- & -- &0.339 \\
26 & -- & -- &1.276 & 58 & -- & -- &0.688 \\
27 & -- & -- &0.959 & 59 & -- & -- &0.190 \\
28 & -- & -- &0.757 & 60 & -- & -- &0.691 \\
29 & -- & -- &1.012 & 61 & -- & -- &0.641 \\
30 & -- & -- &1.004 & 62 & -- & -- &0.831 \\
31 & -- & -- &1.195 & 63 & -- & -- &0.942 \\
32 & -- & -- &1.159 & 64 & -- & -- &0.689 \\
\bottomrule
\end{tabulary}
\caption[EC102--PMTB Efficiency Results]{ \label{tab:EC102--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC102_PMTC_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC102--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.865 & 33 & -- & -- &0.524 \\
02 & -- & -- &1.009 & 34 & -- & -- &1.247 \\
03 & -- & -- &0.815 & 35 & -- & -- &1.070 \\
04 & -- & -- &0.821 & 36 & -- & -- &1.157 \\
05 & -- & -- &0.903 & 37 & -- & -- &0.925 \\
06 & -- & -- &0.859 & 38 & -- & -- &1.091 \\
07 & -- & -- &1.312 & 39 & -- & -- &0.942 \\
08 & -- & -- &1.158 & 40 & -- & -- &1.308 \\
09 & -- & -- &0.863 & 41 & -- & -- &1.041 \\
10 & -- & -- &1.123 & 42 & -- & -- &1.679 \\
11 & -- & -- &1.123 & 43 & -- & -- &1.498 \\
12 & -- & -- &1.216 & 44 & -- & -- &1.115 \\
13 & -- & -- &1.015 & 45 & -- & -- &0.985 \\
14 & -- & -- &1.465 & 46 & -- & -- &1.080 \\
15 & -- & -- &1.425 & 47 & -- & -- &1.262 \\
16 & -- & -- &1.285 & 48 & -- & -- &1.330 \\
17 & -- & -- &1.307 & 49 & -- & -- &1.076 \\
18 & -- & -- &1.172 & 50 & -- & -- &1.547 \\
19 & -- & -- &1.352 & 51 & -- & -- &0.988 \\
20 & -- & -- &1.098 & 52 & -- & -- &1.181 \\
21 & -- & -- &0.986 & 53 & -- & -- &0.358 \\
22 & -- & -- &1.330 & 54 & -- & -- &1.589 \\
23 & -- & -- &1.621 & 55 & -- & -- &1.499 \\
24 & -- & -- &1.576 & 56 & -- & -- &1.366 \\
25 & -- & -- &0.924 & 57 & -- & -- &0.761 \\
26 & -- & -- &1.341 & 58 & -- & -- &1.223 \\
27 & -- & -- &1.227 & 59 & -- & -- &1.238 \\
28 & -- & -- &1.178 & 60 & -- & -- &1.163 \\
29 & -- & -- &1.012 & 61 & -- & -- &1.135 \\
30 & -- & -- &1.301 & 62 & -- & -- &1.064 \\
31 & -- & -- &1.614 & 63 & -- & -- &1.173 \\
32 & -- & -- &1.305 & 64 & -- & -- &0.785 \\
\bottomrule
\end{tabulary}
\caption[EC102--PMTC Efficiency Results]{ \label{tab:EC102--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC102_PMTD_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC102--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.121 & 33 & -- & -- &1.063 \\
02 & -- & -- &1.464 & 34 & -- & -- &1.059 \\
03 & -- & -- &1.329 & 35 & -- & -- &1.067 \\
04 & -- & -- &0.487 & 36 & -- & -- &0.501 \\
05 & -- & -- &0.959 & 37 & -- & -- &0.442 \\
06 & -- & -- &0.980 & 38 & -- & -- &1.683 \\
07 & -- & -- &1.088 & 39 & -- & -- &0.545 \\
08 & -- & -- &0.849 & 40 & -- & -- &0.714 \\
09 & -- & -- &1.218 & 41 & -- & -- &0.320 \\
10 & 0.277 & 0.034 & 1.607 & 42 & -- & -- &0.965 \\
11 & 0.276 & 0.036 & 1.502 & 43 & -- & -- &0.962 \\
12 & -- & -- &1.169 & 44 & -- & -- &0.138 \\
13 & -- & -- &1.014 & 45 & -- & -- &0.860 \\
14 & -- & -- &1.022 & 46 & -- & -- &1.376 \\
15 & -- & -- &1.301 & 47 & -- & -- &0.428 \\
16 & -- & -- &0.868 & 48 & -- & -- &0.712 \\
17 & 0.299 & 0.024 & 1.415 & 49 & -- & -- &0.844 \\
18 & -- & -- &0.953 & 50 & -- & -- &0.879 \\
19 & -- & -- &1.035 & 51 & -- & -- &0.601 \\
20 & -- & -- &1.300 & 52 & -- & -- &0.285 \\
21 & -- & -- &0.768 & 53 & -- & -- &0.714 \\
22 & -- & -- &1.508 & 54 & -- & -- &0.771 \\
23 & -- & -- &0.833 & 55 & -- & -- &0.331 \\
24 & -- & -- &0.620 & 56 & -- & -- &0.284 \\
25 & -- & -- &1.254 & 57 & -- & -- &0.264 \\
26 & -- & -- &1.292 & 58 & -- & -- &0.366 \\
27 & -- & -- &1.007 & 59 & -- & -- &0.423 \\
28 & -- & -- &0.704 & 60 & -- & -- &0.036 \\
29 & -- & -- &1.324 & 61 & -- & -- &0.043 \\
30 & -- & -- &1.027 & 62 & -- & -- &0.045 \\
31 & -- & -- &0.722 & 63 & -- & -- &0.461 \\
32 & -- & -- &0.435 & 64 & -- & -- &0.330 \\
\bottomrule
\end{tabulary}
\caption[EC102--PMTD Efficiency Results]{ \label{tab:EC102--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC103_PMTA_AbsoluteMap_RefPixel056 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC103--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.686 & 33 & -- & -- &0.821 \\
02 & -- & -- &4.799 & 34 & -- & -- &6.379 \\
03 & -- & -- &0.762 & 35 & -- & -- &0.856 \\
04 & -- & -- &1.391 & 36 & -- & -- &0.995 \\
05 & -- & -- &0.626 & 37 & -- & -- &3.221 \\
06 & -- & -- &1.188 & 38 & -- & -- &0.695 \\
07 & -- & -- &0.072 & 39 & -- & -- &0.730 \\
08 & -- & -- &2.956 & 40 & -- & -- &0.604 \\
09 & -- & -- &0.000 & 41 & -- & -- &0.605 \\
10 & -- & -- &1.024 & 42 & -- & -- &0.916 \\
11 & -- & -- &1.776 & 43 & -- & -- &6.695 \\
12 & -- & -- &0.835 & 44 & -- & -- &7.345 \\
13 & -- & -- &11.492 & 45 & -- & -- &1.898 \\
14 & -- & -- &1.234 & 46 & -- & -- &1.228 \\
15 & -- & -- &1.575 & 47 & -- & -- &2.405 \\
16 & -- & -- &0.856 & 48 & -- & -- &0.641 \\
17 & -- & -- &0.502 & 49 & -- & -- &0.094 \\
18 & -- & -- &0.231 & 50 & -- & -- &0.933 \\
19 & -- & -- &3.453 & 51 & -- & -- &0.432 \\
20 & -- & -- &0.120 & 52 & -- & -- &0.334 \\
21 & -- & -- &15.933 & 53 & -- & -- &0.408 \\
22 & -- & -- &4.913 & 54 & -- & -- &0.990 \\
23 & -- & -- &0.619 & 55 & -- & -- &1.219 \\
24 & -- & -- &1.148 & 56 & -- & -- &1.191 \\
25 & -- & -- &2.374 & 57 & -- & -- &0.568 \\
26 & -- & -- &1.350 & 58 & -- & -- &0.216 \\
27 & -- & -- &2.400 & 59 & -- & -- &1.120 \\
28 & -- & -- &0.003 & 60 & -- & -- &1.022 \\
29 & -- & -- &3.948 & 61 & -- & -- &0.684 \\
30 & -- & -- &1.277 & 62 & -- & -- &1.218 \\
31 & -- & -- &0.300 & 63 & -- & -- &1.233 \\
32 & -- & -- &0.485 & 64 & -- & -- &0.445 \\
\bottomrule
\end{tabulary}
\caption[EC103--PMTA Efficiency Results]{ \label{tab:EC103--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC103_PMTB_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC103--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.219 & 33 & -- & -- &0.695 \\
02 & -- & -- &0.452 & 34 & -- & -- &0.082 \\
03 & -- & -- &1.304 & 35 & -- & -- &0.397 \\
04 & -- & -- &0.526 & 36 & -- & -- &0.615 \\
05 & -- & -- &0.762 & 37 & -- & -- &0.942 \\
06 & -- & -- &1.292 & 38 & -- & -- &0.408 \\
07 & -- & -- &1.883 & 39 & -- & -- &0.873 \\
08 & -- & -- &8.166 & 40 & -- & -- &0.887 \\
09 & -- & -- &0.302 & 41 & -- & -- &2.134 \\
10 & -- & -- &0.358 & 42 & -- & -- &1.067 \\
11 & -- & -- &0.184 & 43 & -- & -- &0.236 \\
12 & -- & -- &0.907 & 44 & -- & -- &1.357 \\
13 & -- & -- &1.939 & 45 & -- & -- &0.333 \\
14 & -- & -- &0.466 & 46 & -- & -- &0.885 \\
15 & -- & -- &0.444 & 47 & -- & -- &0.659 \\
16 & -- & -- &2.428 & 48 & -- & -- &0.536 \\
17 & 0.009 & 0.052 & 0.377 & 49 & -- & -- &0.650 \\
18 & -- & -- &1.230 & 50 & -- & -- &0.367 \\
19 & -- & -- &0.245 & 51 & -- & -- &0.720 \\
20 & -- & -- &1.331 & 52 & -- & -- &0.661 \\
21 & -- & -- &0.470 & 53 & -- & -- &1.312 \\
22 & -- & -- &1.504 & 54 & -- & -- &1.429 \\
23 & -- & -- &1.885 & 55 & -- & -- &0.709 \\
24 & -- & -- &0.542 & 56 & -- & -- &0.662 \\
25 & -- & -- &1.373 & 57 & -- & -- &0.455 \\
26 & -- & -- &0.748 & 58 & -- & -- &0.655 \\
27 & -- & -- &1.366 & 59 & -- & -- &0.788 \\
28 & -- & -- &0.177 & 60 & -- & -- &0.845 \\
29 & -- & -- &0.584 & 61 & -- & -- &0.461 \\
30 & -- & -- &0.488 & 62 & -- & -- &0.554 \\
31 & -- & -- &2.871 & 63 & -- & -- &0.719 \\
32 & -- & -- &0.887 & 64 & -- & -- &0.000 \\
\bottomrule
\end{tabulary}
\caption[EC103--PMTB Efficiency Results]{ \label{tab:EC103--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC103_PMTC_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC103--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &44.635 & 33 & -- & -- &0.289 \\
02 & -- & -- &20.737 & 34 & -- & -- &0.224 \\
03 & -- & -- &1.074 & 35 & -- & -- &0.499 \\
04 & -- & -- &0.202 & 36 & -- & -- &0.903 \\
05 & -- & -- &1.328 & 37 & -- & -- &0.988 \\
06 & -- & -- &109.380 & 38 & -- & -- &1.123 \\
07 & -- & -- &0.716 & 39 & -- & -- &1.158 \\
08 & -- & -- &0.673 & 40 & -- & -- &0.906 \\
09 & -- & -- &2.413 & 41 & -- & -- &0.122 \\
10 & -- & -- &1.372 & 42 & -- & -- &2.218 \\
11 & -- & -- &0.579 & 43 & -- & -- &0.842 \\
12 & -- & -- &1.038 & 44 & -- & -- &0.528 \\
13 & -- & -- &0.584 & 45 & -- & -- &1.164 \\
14 & -- & -- &0.810 & 46 & -- & -- &0.910 \\
15 & -- & -- &0.726 & 47 & -- & -- &0.418 \\
16 & -- & -- &0.721 & 48 & -- & -- &0.714 \\
17 & -- & -- &0.076 & 49 & -- & -- &0.106 \\
18 & -- & -- &0.779 & 50 & -- & -- &1.543 \\
19 & -- & -- &1.154 & 51 & -- & -- &1.318 \\
20 & -- & -- &0.695 & 52 & -- & -- &0.712 \\
21 & -- & -- &0.910 & 53 & -- & -- &0.401 \\
22 & 0.284 & 0.021 & 1.769 & 54 & 0.291 & 0.035 & 1.358 \\
23 & -- & -- &0.417 & 55 & -- & -- &1.361 \\
24 & -- & -- &0.606 & 56 & -- & -- &0.593 \\
25 & -- & -- &0.232 & 57 & -- & -- &0.622 \\
26 & -- & -- &0.855 & 58 & -- & -- &0.026 \\
27 & -- & -- &1.048 & 59 & -- & -- &1.902 \\
28 & -- & -- &0.544 & 60 & -- & -- &2.621 \\
29 & -- & -- &0.589 & 61 & -- & -- &0.596 \\
30 & -- & -- &1.395 & 62 & -- & -- &0.069 \\
31 & -- & -- &0.964 & 63 & -- & -- &2.068 \\
32 & -- & -- &0.211 & 64 & -- & -- &1.515 \\
\bottomrule
\end{tabulary}
\caption[EC103--PMTC Efficiency Results]{ \label{tab:EC103--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC103_PMTD_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC103--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.006 & 33 & -- & -- &1.146 \\
02 & -- & -- &1.256 & 34 & -- & -- &0.413 \\
03 & -- & -- &1.287 & 35 & -- & -- &1.325 \\
04 & -- & -- &0.764 & 36 & -- & -- &1.173 \\
05 & -- & -- &0.956 & 37 & -- & -- &0.464 \\
06 & -- & -- &0.381 & 38 & -- & -- &1.286 \\
07 & -- & -- &0.571 & 39 & 0.230 & 0.035 & 1.560 \\
08 & -- & -- &0.275 & 40 & -- & -- &1.405 \\
09 & -- & -- &1.173 & 41 & -- & -- &0.981 \\
10 & 0.230 & 0.034 & 1.457 & 42 & -- & -- &0.769 \\
11 & 0.225 & 0.033 & 1.735 & 43 & 0.227 & 0.035 & 1.473 \\
12 & 0.227 & 0.036 & 1.484 & 44 & -- & -- &0.820 \\
13 & -- & -- &0.811 & 45 & -- & -- &0.980 \\
14 & -- & -- &0.539 & 46 & 0.219 & 0.034 & 1.503 \\
15 & -- & -- &0.384 & 47 & 0.223 & 0.035 & 1.414 \\
16 & -- & -- &0.421 & 48 & -- & -- &1.147 \\
17 & 0.282 & 0.024 & 1.378 & 49 & -- & -- &0.860 \\
18 & -- & -- &1.098 & 50 & -- & -- &1.217 \\
19 & 0.237 & 0.038 & 1.392 & 51 & -- & -- &0.617 \\
20 & -- & -- &0.912 & 52 & -- & -- &1.060 \\
21 & -- & -- &1.210 & 53 & -- & -- &1.334 \\
22 & -- & -- &0.739 & 54 & 0.231 & 0.035 & 1.498 \\
23 & -- & -- &0.940 & 55 & 0.206 & 0.030 & 1.697 \\
24 & -- & -- &0.244 & 56 & -- & -- &1.094 \\
25 & 0.262 & 0.038 & 1.345 & 57 & -- & -- &1.221 \\
26 & -- & -- &0.899 & 58 & -- & -- &0.899 \\
27 & -- & -- &1.209 & 59 & -- & -- &1.110 \\
28 & -- & -- &0.992 & 60 & -- & -- &1.045 \\
29 & -- & -- &0.918 & 61 & -- & -- &1.569 \\
30 & -- & -- &1.301 & 62 & -- & -- &1.447 \\
31 & -- & -- &1.030 & 63 & -- & -- &1.306 \\
32 & -- & -- &1.195 & 64 & -- & -- &0.843 \\
\bottomrule
\end{tabulary}
\caption[EC103--PMTD Efficiency Results]{ \label{tab:EC103--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC105_PMTA_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC105--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.056 & 33 & -- & -- &0.382 \\
02 & -- & -- &1.245 & 34 & 0.264 & 0.030 & 1.638 \\
03 & -- & -- &1.340 & 35 & 0.281 & 0.033 & 1.536 \\
04 & 0.312 & 0.032 & 1.468 & 36 & 0.262 & 0.028 & 1.934 \\
05 & -- & -- &0.978 & 37 & 0.278 & 0.033 & 1.581 \\
06 & 0.312 & 0.032 & 1.461 & 38 & 0.260 & 0.027 & 1.873 \\
07 & -- & -- &1.370 & 39 & 0.276 & 0.035 & 1.387 \\
08 & -- & -- &1.124 & 40 & 0.277 & 0.034 & 1.294 \\
09 & -- & -- &0.865 & 41 & 0.294 & 0.033 & 1.480 \\
10 & 0.262 & 0.032 & 1.325 & 42 & 0.256 & 0.027 & 1.981 \\
11 & 0.274 & 0.033 & 1.606 & 43 & 0.258 & 0.028 & 1.802 \\
12 & 0.266 & 0.032 & 1.698 & 44 & 0.257 & 0.028 & 1.848 \\
13 & 0.272 & 0.034 & 1.357 & 45 & -- & -- &1.247 \\
14 & 0.268 & 0.030 & 1.689 & 46 & 0.271 & 0.032 & 1.394 \\
15 & 0.259 & 0.030 & 1.557 & 47 & 0.266 & 0.030 & 1.651 \\
16 & 0.270 & 0.035 & 1.529 & 48 & 0.270 & 0.032 & 1.252 \\
17 & 0.283 & 0.034 & 1.377 & 49 & -- & -- &0.788 \\
18 & 0.252 & 0.027 & 1.923 & 50 & -- & -- &1.241 \\
19 & 0.262 & 0.031 & 1.442 & 51 & -- & -- &1.230 \\
20 & -- & -- &1.372 & 52 & 0.266 & 0.031 & 1.498 \\
21 & 0.287 & 0.034 & 1.526 & 53 & -- & -- &0.728 \\
22 & 0.249 & 0.021 & 2.737 & 54 & 0.274 & 0.030 & 1.795 \\
23 & -- & -- &0.857 & 55 & -- & -- &1.260 \\
24 & 0.269 & 0.031 & 1.656 & 56 & -- & -- &1.238 \\
25 & 0.286 & 0.033 & 1.504 & 57 & -- & -- &0.720 \\
26 & 0.251 & 0.027 & 1.907 & 58 & -- & -- &0.937 \\
27 & 0.258 & 0.028 & 1.999 & 59 & -- & -- &0.780 \\
28 & 0.260 & 0.026 & 2.209 & 60 & -- & -- &0.994 \\
29 & 0.270 & 0.030 & 1.624 & 61 & -- & -- &1.035 \\
30 & 0.259 & 0.026 & 2.354 & 62 & -- & -- &0.840 \\
31 & 0.254 & 0.026 & 2.264 & 63 & -- & -- &0.816 \\
32 & 0.252 & 0.028 & 1.526 & 64 & -- & -- &0.718 \\
\bottomrule
\end{tabulary}
\caption[EC105--PMTA Efficiency Results]{ \label{tab:EC105--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC105_PMTB_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC105--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.728 & 33 & -- & -- &1.134 \\
02 & -- & -- &0.899 & 34 & -- & -- &0.206 \\
03 & -- & -- &1.220 & 35 & 0.209 & 0.032 & 1.396 \\
04 & -- & -- &0.634 & 36 & -- & -- &0.911 \\
05 & -- & -- &1.250 & 37 & -- & -- &1.073 \\
06 & -- & -- &0.781 & 38 & -- & -- &1.481 \\
07 & -- & -- &0.664 & 39 & 0.202 & 0.027 & 1.775 \\
08 & -- & -- &0.444 & 40 & -- & -- &1.202 \\
09 & -- & -- &0.906 & 41 & 0.210 & 0.029 & 1.689 \\
10 & -- & -- &0.945 & 42 & 0.218 & 0.033 & 1.496 \\
11 & 0.219 & 0.032 & 1.339 & 43 & 0.225 & 0.035 & 1.505 \\
12 & 0.207 & 0.027 & 1.764 & 44 & -- & -- &0.739 \\
13 & -- & -- &1.018 & 45 & 0.196 & 0.027 & 1.825 \\
14 & -- & -- &0.823 & 46 & 0.206 & 0.029 & 1.844 \\
15 & -- & -- &0.527 & 47 & 0.194 & 0.026 & 1.968 \\
16 & -- & -- &0.833 & 48 & 0.219 & 0.030 & 1.514 \\
17 & -- & -- &0.906 & 49 & -- & -- &1.178 \\
18 & -- & -- &0.985 & 50 & -- & -- &1.146 \\
19 & 0.209 & 0.031 & 1.468 & 51 & -- & -- &0.804 \\
20 & -- & -- &1.280 & 52 & -- & -- &0.420 \\
21 & 0.210 & 0.028 & 1.777 & 53 & 0.220 & 0.035 & 1.261 \\
22 & 0.241 & 0.021 & 2.006 & 54 & -- & -- &1.048 \\
23 & -- & -- &1.260 & 55 & 0.228 & 0.034 & 1.418 \\
24 & -- & -- &0.381 & 56 & -- & -- &1.176 \\
25 & -- & -- &0.918 & 57 & -- & -- &0.921 \\
26 & -- & -- &1.063 & 58 & -- & -- &0.789 \\
27 & -- & -- &0.985 & 59 & -- & -- &0.391 \\
28 & -- & -- &0.894 & 60 & -- & -- &0.430 \\
29 & -- & -- &1.177 & 61 & -- & -- &0.986 \\
30 & -- & -- &1.267 & 62 & -- & -- &0.852 \\
31 & -- & -- &1.110 & 63 & -- & -- &1.019 \\
32 & -- & -- &1.059 & 64 & -- & -- &0.363 \\
\bottomrule
\end{tabulary}
\caption[EC105--PMTB Efficiency Results]{ \label{tab:EC105--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC105_PMTC_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC105--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.922 & 33 & 0.276 & 0.033 & 1.322 \\
02 & 0.299 & 0.029 & 1.361 & 34 & 0.244 & 0.026 & 2.174 \\
03 & 0.322 & 0.032 & 1.182 & 35 & 0.238 & 0.026 & 2.193 \\
04 & 0.298 & 0.031 & 1.390 & 36 & 0.231 & 0.025 & 2.409 \\
05 & -- & -- &1.062 & 37 & 0.241 & 0.026 & 2.295 \\
06 & 0.303 & 0.033 & 1.427 & 38 & 0.236 & 0.025 & 2.408 \\
07 & 0.294 & 0.032 & 1.504 & 39 & 0.247 & 0.026 & 2.419 \\
08 & 0.279 & 0.035 & 1.242 & 40 & 0.259 & 0.028 & 1.468 \\
09 & 0.298 & 0.033 & 1.338 & 41 & 0.259 & 0.027 & 1.778 \\
10 & 0.237 & 0.024 & 2.980 & 42 & 0.240 & 0.026 & 2.150 \\
11 & 0.244 & 0.025 & 2.541 & 43 & 0.237 & 0.025 & 2.467 \\
12 & 0.236 & 0.025 & 2.513 & 44 & 0.235 & 0.024 & 2.433 \\
13 & 0.261 & 0.031 & 1.921 & 45 & 0.241 & 0.027 & 2.240 \\
14 & 0.241 & 0.025 & 2.707 & 46 & 0.229 & 0.024 & 2.841 \\
15 & 0.243 & 0.025 & 2.525 & 47 & 0.238 & 0.024 & 2.541 \\
16 & 0.256 & 0.030 & 1.813 & 48 & 0.267 & 0.032 & 1.250 \\
17 & 0.272 & 0.021 & 2.112 & 49 & -- & -- &1.386 \\
18 & 0.240 & 0.024 & 2.982 & 50 & 0.258 & 0.027 & 1.818 \\
19 & 0.231 & 0.025 & 2.696 & 51 & 0.250 & 0.026 & 1.878 \\
20 & 0.231 & 0.025 & 2.230 & 52 & 0.242 & 0.026 & 2.514 \\
21 & 0.240 & 0.025 & 2.532 & 53 & 0.230 & 0.027 & 1.572 \\
22 & 0.232 & 0.024 & 3.061 & 54 & 0.234 & 0.024 & 2.964 \\
23 & -- & -- &1.031 & 55 & 0.242 & 0.025 & 2.453 \\
24 & 0.251 & 0.026 & 1.892 & 56 & 0.264 & 0.033 & 1.178 \\
25 & 0.271 & 0.029 & 1.732 & 57 & -- & -- &0.721 \\
26 & 0.243 & 0.026 & 2.732 & 58 & -- & -- &1.066 \\
27 & 0.232 & 0.024 & 2.854 & 59 & -- & -- &1.189 \\
28 & 0.233 & 0.025 & 2.817 & 60 & 0.281 & 0.034 & 1.207 \\
29 & 0.235 & 0.026 & 2.410 & 61 & 0.284 & 0.034 & 1.297 \\
30 & 0.241 & 0.025 & 2.818 & 62 & 0.288 & 0.035 & 1.292 \\
31 & 0.243 & 0.025 & 2.851 & 63 & -- & -- &1.192 \\
32 & 0.260 & 0.027 & 1.816 & 64 & -- & -- &0.657 \\
\bottomrule
\end{tabulary}
\caption[EC105--PMTC Efficiency Results]{ \label{tab:EC105--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC105_PMTD_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC105--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.219 & 0.028 & 1.893 & 33 & 0.249 & 0.026 & 2.130 \\
02 & 0.225 & 0.026 & 2.537 & 34 & -- & -- &1.148 \\
03 & 0.231 & 0.026 & 2.509 & 35 & 0.225 & 0.027 & 2.423 \\
04 & -- & -- &1.182 & 36 & 0.228 & 0.028 & 1.876 \\
05 & 0.261 & 0.031 & 1.595 & 37 & 0.243 & 0.036 & 1.494 \\
06 & 0.262 & 0.030 & 1.781 & 38 & 0.235 & 0.032 & 1.627 \\
07 & 0.250 & 0.034 & 1.371 & 39 & 0.235 & 0.027 & 2.181 \\
08 & -- & -- &1.600 & 40 & -- & -- &1.111 \\
09 & 0.244 & 0.026 & 2.717 & 41 & 0.245 & 0.026 & 2.329 \\
10 & 0.227 & 0.025 & 2.827 & 42 & 0.218 & 0.026 & 2.203 \\
11 & 0.232 & 0.025 & 3.198 & 43 & 0.222 & 0.027 & 2.172 \\
12 & 0.231 & 0.025 & 2.900 & 44 & 0.223 & 0.027 & 2.266 \\
13 & 0.235 & 0.027 & 2.432 & 45 & 0.220 & 0.026 & 2.273 \\
14 & 0.228 & 0.026 & 2.660 & 46 & 0.214 & 0.026 & 2.068 \\
15 & 0.231 & 0.027 & 2.236 & 47 & 0.229 & 0.028 & 2.083 \\
16 & -- & -- &0.657 & 48 & 0.253 & 0.035 & 1.251 \\
17 & 0.247 & 0.026 & 2.455 & 49 & 0.246 & 0.029 & 1.998 \\
18 & 0.229 & 0.026 & 2.565 & 50 & 0.227 & 0.027 & 1.965 \\
19 & 0.224 & 0.026 & 2.515 & 51 & 0.235 & 0.031 & 1.745 \\
20 & 0.225 & 0.027 & 2.057 & 52 & 0.238 & 0.033 & 1.608 \\
21 & 0.230 & 0.027 & 2.161 & 53 & 0.229 & 0.027 & 1.965 \\
22 & 0.235 & 0.022 & 1.870 & 54 & 0.246 & 0.033 & 1.540 \\
23 & 0.240 & 0.030 & 1.782 & 55 & 0.243 & 0.032 & 1.880 \\
24 & -- & -- &5.913 & 56 & -- & -- &0.854 \\
25 & 0.243 & 0.026 & 2.589 & 57 & -- & -- &1.119 \\
26 & 0.226 & 0.026 & 2.667 & 58 & -- & -- &1.078 \\
27 & 0.225 & 0.026 & 2.381 & 59 & -- & -- &1.135 \\
28 & -- & -- &0.554 & 60 & -- & -- &1.153 \\
29 & 0.228 & 0.027 & 2.220 & 61 & -- & -- &1.160 \\
30 & 0.233 & 0.027 & 2.197 & 62 & -- & -- &0.900 \\
31 & 0.233 & 0.026 & 2.418 & 63 & -- & -- &0.546 \\
32 & -- & -- &1.046 & 64 & -- & -- &0.560 \\
\bottomrule
\end{tabulary}
\caption[EC105--PMTD Efficiency Results]{ \label{tab:EC105--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC106_PMTA_AbsoluteMap_RefPixel051 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC106--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.288 & 0.028 & 2.242 & 33 & 0.261 & 0.028 & 1.913 \\
02 & 0.264 & 0.026 & 2.930 & 34 & 0.228 & 0.029 & 1.681 \\
03 & 0.259 & 0.026 & 2.240 & 35 & -- & -- &0.007 \\
04 & 0.249 & 0.026 & 2.402 & 36 & 0.234 & 0.034 & 1.318 \\
05 & 0.272 & 0.028 & 2.224 & 37 & -- & -- &1.313 \\
06 & 0.271 & 0.027 & 2.357 & 38 & 0.238 & 0.033 & 1.476 \\
07 & 0.288 & 0.029 & 2.078 & 39 & 0.244 & 0.033 & 1.631 \\
08 & 0.282 & 0.036 & 1.444 & 40 & 0.244 & 0.028 & 1.824 \\
09 & 0.242 & 0.026 & 2.029 & 41 & 0.258 & 0.028 & 2.300 \\
10 & 0.223 & 0.026 & 2.517 & 42 & 0.224 & 0.026 & 2.311 \\
11 & 0.221 & 0.026 & 2.669 & 43 & 0.243 & 0.036 & 1.419 \\
12 & 0.226 & 0.027 & 2.290 & 44 & 0.220 & 0.029 & 1.672 \\
13 & 0.233 & 0.029 & 2.219 & 45 & -- & -- &1.493 \\
14 & 0.244 & 0.031 & 2.051 & 46 & -- & -- &0.324 \\
15 & 0.228 & 0.027 & 1.750 & 47 & 0.233 & 0.029 & 1.937 \\
16 & 0.246 & 0.031 & 1.612 & 48 & 0.233 & 0.029 & 1.776 \\
17 & 0.259 & 0.026 & 2.585 & 49 & 0.261 & 0.028 & 2.194 \\
18 & 0.231 & 0.027 & 2.264 & 50 & 0.235 & 0.032 & 1.836 \\
19 & 0.236 & 0.030 & 1.880 & 51 & 0.240 & 0.022 & 1.906 \\
20 & -- & -- &1.127 & 52 & 0.233 & 0.029 & 2.006 \\
21 & 0.250 & 0.036 & 1.427 & 53 & -- & -- &1.252 \\
22 & 0.237 & 0.031 & 1.857 & 54 & 0.232 & 0.028 & 2.233 \\
23 & 0.234 & 0.029 & 1.895 & 55 & 0.225 & 0.027 & 2.152 \\
24 & 0.240 & 0.028 & 1.972 & 56 & 0.232 & 0.028 & 2.026 \\
25 & 0.252 & 0.027 & 2.335 & 57 & -- & -- &1.570 \\
26 & 0.221 & 0.027 & 2.180 & 58 & 0.270 & 0.027 & 1.933 \\
27 & 0.233 & 0.029 & 1.938 & 59 & 0.280 & 0.033 & 1.643 \\
28 & 0.236 & 0.033 & 1.567 & 60 & 0.291 & 0.036 & 1.416 \\
29 & 0.228 & 0.033 & 1.404 & 61 & 0.292 & 0.033 & 1.755 \\
30 & 0.247 & 0.034 & 1.368 & 62 & 0.268 & 0.032 & 1.519 \\
31 & 0.232 & 0.028 & 1.755 & 63 & 0.285 & 0.031 & 1.592 \\
32 & 0.245 & 0.029 & 2.012 & 64 & 0.259 & 0.035 & 1.402 \\
\bottomrule
\end{tabulary}
\caption[EC106--PMTA Efficiency Results]{ \label{tab:EC106--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC106_PMTB_AbsoluteMap_RefPixel033 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC106--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.015 & 33 & 0.213 & 0.021 & 2.214 \\
02 & -- & -- &1.080 & 34 & 0.186 & 0.029 & 1.887 \\
03 & -- & -- &1.166 & 35 & 0.190 & 0.027 & 1.951 \\
04 & -- & -- &0.752 & 36 & 0.181 & 0.026 & 1.825 \\
05 & -- & -- &1.027 & 37 & 0.179 & 0.029 & 1.661 \\
06 & -- & -- &1.109 & 38 & 0.184 & 0.028 & 1.707 \\
07 & -- & -- &1.206 & 39 & 0.197 & 0.027 & 1.644 \\
08 & -- & -- &0.739 & 40 & 0.198 & 0.031 & 1.241 \\
09 & 0.236 & 0.027 & 2.246 & 41 & 0.211 & 0.026 & 2.316 \\
10 & 0.205 & 0.026 & 2.482 & 42 & 0.191 & 0.027 & 1.706 \\
11 & 0.200 & 0.025 & 2.686 & 43 & 0.183 & 0.028 & 1.767 \\
12 & 0.200 & 0.026 & 2.307 & 44 & 0.180 & 0.028 & 1.784 \\
13 & 0.196 & 0.026 & 2.244 & 45 & 0.190 & 0.027 & 1.631 \\
14 & 0.212 & 0.026 & 1.988 & 46 & 0.190 & 0.030 & 1.950 \\
15 & 0.213 & 0.026 & 1.942 & 47 & 0.187 & 0.028 & 1.639 \\
16 & 0.203 & 0.033 & 1.340 & 48 & -- & -- &1.212 \\
17 & 0.222 & 0.025 & 2.122 & 49 & 0.210 & 0.028 & 2.072 \\
18 & 0.187 & 0.026 & 2.092 & 50 & 0.183 & 0.030 & 1.952 \\
19 & 0.192 & 0.026 & 2.207 & 51 & 0.184 & 0.027 & 2.053 \\
20 & 0.192 & 0.028 & 2.071 & 52 & 0.172 & 0.028 & 1.828 \\
21 & 0.188 & 0.027 & 2.240 & 53 & 0.183 & 0.027 & 1.702 \\
22 & 0.202 & 0.027 & 2.192 & 54 & 0.180 & 0.027 & 1.643 \\
23 & 0.207 & 0.026 & 1.882 & 55 & 0.185 & 0.027 & 1.613 \\
24 & 0.205 & 0.033 & 1.487 & 56 & 0.158 & 0.035 & 1.108 \\
25 & 0.222 & 0.026 & 2.067 & 57 & -- & -- &1.097 \\
26 & 0.180 & 0.027 & 2.370 & 58 & -- & -- &0.950 \\
27 & -- & -- &0.949 & 59 & -- & -- &0.798 \\
28 & 0.182 & 0.027 & 1.967 & 60 & -- & -- &0.995 \\
29 & 0.191 & 0.027 & 2.333 & 61 & -- & -- &1.144 \\
30 & 0.196 & 0.027 & 1.846 & 62 & -- & -- &0.928 \\
31 & 0.201 & 0.027 & 1.856 & 63 & -- & -- &0.966 \\
32 & 0.209 & 0.029 & 1.207 & 64 & -- & -- &1.366 \\
\bottomrule
\end{tabulary}
\caption[EC106--PMTB Efficiency Results]{ \label{tab:EC106--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC106_PMTC_AbsoluteMap_RefPixel051 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC106--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.021 & 33 & -- & -- &1.138 \\
02 & -- & -- &1.594 & 34 & -- & -- &2.153 \\
03 & -- & -- &1.584 & 35 & -- & -- &1.697 \\
04 & -- & -- &1.671 & 36 & -- & -- &2.048 \\
05 & -- & -- &1.482 & 37 & -- & -- &1.842 \\
06 & -- & -- &1.550 & 38 & -- & -- &2.209 \\
07 & -- & -- &1.939 & 39 & -- & -- &2.203 \\
08 & -- & -- &0.648 & 40 & -- & -- &2.201 \\
09 & -- & -- &1.581 & 41 & -- & -- &1.991 \\
10 & -- & -- &2.811 & 42 & -- & -- &2.744 \\
11 & -- & -- &2.922 & 43 & -- & -- &2.208 \\
12 & -- & -- &2.869 & 44 & -- & -- &2.242 \\
13 & -- & -- &2.426 & 45 & -- & -- &1.550 \\
14 & -- & -- &2.311 & 46 & -- & -- &0.432 \\
15 & -- & -- &2.114 & 47 & -- & -- &2.486 \\
16 & -- & -- &1.562 & 48 & -- & -- &2.118 \\
17 & -- & -- &2.305 & 49 & -- & -- &2.021 \\
18 & -- & -- &2.762 & 50 & -- & -- &2.116 \\
19 & -- & -- &2.196 & 51 & -- & -- &0.000 \\
20 & -- & -- &1.703 & 52 & -- & -- &2.066 \\
21 & -- & -- &2.024 & 53 & -- & -- &1.089 \\
22 & -- & -- &2.457 & 54 & -- & -- &2.442 \\
23 & -- & -- &2.124 & 55 & -- & -- &2.507 \\
24 & -- & -- &2.137 & 56 & -- & -- &2.229 \\
25 & -- & -- &1.585 & 57 & -- & -- &1.069 \\
26 & -- & -- &1.853 & 58 & -- & -- &1.068 \\
27 & -- & -- &2.392 & 59 & -- & -- &0.444 \\
28 & -- & -- &2.109 & 60 & -- & -- &0.768 \\
29 & -- & -- &2.048 & 61 & -- & -- &1.271 \\
30 & -- & -- &1.752 & 62 & -- & -- &1.464 \\
31 & -- & -- &2.015 & 63 & -- & -- &2.013 \\
32 & -- & -- &2.156 & 64 & -- & -- &1.455 \\
\bottomrule
\end{tabulary}
\caption[EC106--PMTC Efficiency Results]{ \label{tab:EC106--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC106_PMTD_AbsoluteMap_RefPixel033 <==
\begin{table}
\centering
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC106--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.244 & 0.025 & 2.899 & 33 & 0.229 & 0.021 & 3.190 \\
02 & 0.246 & 0.025 & 2.753 & 34 & 0.200 & 0.025 & 2.749 \\
03 & 0.244 & 0.025 & 2.909 & 35 & 0.205 & 0.025 & 3.079 \\
04 & 0.261 & 0.031 & 2.227 & 36 & 0.203 & 0.025 & 2.917 \\
05 & 0.244 & 0.025 & 2.522 & 37 & 0.195 & 0.025 & 2.501 \\
06 & -- & -- &1.270 & 38 & 0.202 & 0.025 & 2.618 \\
07 & -- & -- &0.715 & 39 & 0.206 & 0.025 & 2.532 \\
08 & -- & -- &0.360 & 40 & 0.220 & 0.025 & 2.445 \\
09 & 0.233 & 0.024 & 3.359 & 41 & 0.224 & 0.025 & 3.033 \\
10 & 0.212 & 0.025 & 3.540 & 42 & 0.206 & 0.025 & 2.640 \\
11 & 0.212 & 0.025 & 3.658 & 43 & 0.204 & 0.025 & 2.395 \\
12 & 0.211 & 0.025 & 3.346 & 44 & 0.205 & 0.025 & 2.841 \\
13 & 0.212 & 0.027 & 1.866 & 45 & 0.201 & 0.026 & 2.772 \\
14 & -- & -- &1.173 & 46 & 0.203 & 0.025 & 2.833 \\
15 & -- & -- &0.858 & 47 & 0.198 & 0.025 & 2.566 \\
16 & -- & -- &0.808 & 48 & 0.210 & 0.026 & 2.502 \\
17 & 0.234 & 0.025 & 3.199 & 49 & 0.225 & 0.026 & 3.146 \\
18 & 0.203 & 0.025 & 3.448 & 50 & 0.204 & 0.025 & 2.839 \\
19 & 0.211 & 0.025 & 3.118 & 51 & 0.201 & 0.025 & 2.464 \\
20 & 0.213 & 0.025 & 2.893 & 52 & 0.200 & 0.025 & 2.335 \\
21 & 0.212 & 0.025 & 2.957 & 53 & 0.205 & 0.025 & 2.578 \\
22 & 0.220 & 0.030 & 1.982 & 54 & 0.204 & 0.025 & 2.584 \\
23 & 0.224 & 0.032 & 1.702 & 55 & 0.210 & 0.025 & 2.673 \\
24 & -- & -- &1.252 & 56 & 0.198 & 0.027 & 1.856 \\
25 & 0.234 & 0.025 & 3.324 & 57 & 0.230 & 0.028 & 2.060 \\
26 & 0.216 & 0.025 & 3.197 & 58 & 0.225 & 0.027 & 1.610 \\
27 & -- & -- &1.471 & 59 & -- & -- &1.250 \\
28 & 0.206 & 0.025 & 2.603 & 60 & 0.225 & 0.028 & 1.831 \\
29 & 0.213 & 0.028 & 2.257 & 61 & 0.227 & 0.027 & 2.486 \\
30 & 0.218 & 0.031 & 1.826 & 62 & 0.217 & 0.026 & 2.101 \\
31 & -- & -- &1.384 & 63 & 0.213 & 0.025 & 2.352 \\
32 & 0.218 & 0.029 & 1.498 & 64 & -- & -- &1.251 \\
\bottomrule
\end{tabulary}
\caption[EC106--PMTD Efficiency Results]{ \label{tab:EC106--PMTD EffResults}}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC107_PMTA_AbsoluteMap_RefPixel033 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC107--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &0.496 & 33 & 0.325 & 0.028 & 1.328 \\
02 & -- & -- &1.117 & 34 & 0.279 & 0.031 & 2.935 \\
03 & -- & -- &1.131 & 35 & 0.281 & 0.031 & 2.722 \\
04 & -- & -- &1.347 & 36 & 0.295 & 0.032 & 2.586 \\
05 & -- & -- &1.223 & 37 & 0.283 & 0.031 & 2.410 \\
06 & -- & -- &0.984 & 38 & 0.303 & 0.031 & 2.619 \\
07 & 0.357 & 0.039 & 1.308 & 39 & 0.273 & 0.031 & 2.128 \\
08 & -- & -- &0.362 & 40 & 0.343 & 0.034 & 1.639 \\
09 & -- & -- &1.273 & 41 & 0.307 & 0.031 & 2.922 \\
10 & 0.271 & 0.031 & 2.582 & 42 & 0.293 & 0.031 & 3.326 \\
11 & 0.282 & 0.031 & 2.238 & 43 & 0.286 & 0.031 & 2.909 \\
12 & 0.260 & 0.031 & 2.164 & 44 & 0.292 & 0.031 & 2.438 \\
13 & 0.268 & 0.031 & 2.123 & 45 & 0.296 & 0.033 & 2.372 \\
14 & 0.281 & 0.031 & 2.514 & 46 & 0.288 & 0.032 & 2.573 \\
15 & 0.280 & 0.032 & 1.998 & 47 & 0.292 & 0.031 & 2.840 \\
16 & -- & -- &1.082 & 48 & 0.324 & 0.034 & 1.874 \\
17 & 0.314 & 0.031 & 2.504 & 49 & 0.330 & 0.031 & 2.765 \\
18 & 0.295 & 0.032 & 2.322 & 50 & 0.293 & 0.031 & 2.929 \\
19 & 0.279 & 0.031 & 2.589 & 51 & 0.302 & 0.032 & 2.248 \\
20 & -- & -- &0.811 & 52 & 0.298 & 0.031 & 2.906 \\
21 & 0.293 & 0.032 & 2.646 & 53 & -- & -- &1.544 \\
22 & 0.281 & 0.031 & 2.427 & 54 & 0.300 & 0.031 & 2.925 \\
23 & 0.290 & 0.032 & 2.427 & 55 & 0.310 & 0.031 & 2.636 \\
24 & 0.350 & 0.036 & 1.557 & 56 & 0.312 & 0.033 & 1.655 \\
25 & 0.306 & 0.031 & 2.409 & 57 & -- & -- &1.115 \\
26 & 0.281 & 0.031 & 2.896 & 58 & 0.348 & 0.033 & 2.054 \\
27 & 0.292 & 0.031 & 2.848 & 59 & 0.351 & 0.033 & 2.115 \\
28 & 0.295 & 0.032 & 2.563 & 60 & 0.348 & 0.032 & 2.286 \\
29 & 0.293 & 0.031 & 2.534 & 61 & 0.333 & 0.031 & 2.614 \\
30 & 0.296 & 0.031 & 2.885 & 62 & 0.323 & 0.031 & 2.552 \\
31 & 0.287 & 0.031 & 2.131 & 63 & 0.343 & 0.032 & 2.478 \\
32 & 0.341 & 0.037 & 1.538 & 64 & -- & -- &0.139 \\
\bottomrule
\end{tabulary}
\caption[EC107--PMTA Efficiency Results]{ \label{tab:EC107--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC107_PMTB_AbsoluteMap_RefPixel033 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC107--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.229 & 0.026 & 2.261 & 33 & 0.222 & 0.021 & 2.812 \\
02 & 0.232 & 0.025 & 2.611 & 34 & 0.218 & 0.026 & 2.455 \\
03 & 0.230 & 0.025 & 2.553 & 35 & 0.217 & 0.025 & 2.440 \\
04 & -- & -- &1.085 & 36 & 0.220 & 0.026 & 2.314 \\
05 & 0.255 & 0.030 & 2.230 & 37 & -- & -- &1.377 \\
06 & 0.232 & 0.026 & 1.868 & 38 & 0.214 & 0.026 & 2.316 \\
07 & 0.236 & 0.026 & 2.054 & 39 & 0.221 & 0.027 & 2.058 \\
08 & 0.234 & 0.030 & 1.748 & 40 & 0.225 & 0.026 & 1.802 \\
09 & 0.213 & 0.026 & 2.786 & 41 & 0.210 & 0.026 & 2.223 \\
10 & 0.226 & 0.025 & 3.026 & 42 & 0.233 & 0.029 & 2.304 \\
11 & 0.201 & 0.025 & 2.956 & 43 & 0.216 & 0.026 & 2.113 \\
12 & 0.219 & 0.025 & 2.372 & 44 & 0.221 & 0.027 & 2.158 \\
13 & 0.217 & 0.025 & 2.877 & 45 & 0.218 & 0.025 & 2.434 \\
14 & 0.216 & 0.025 & 2.621 & 46 & 0.212 & 0.025 & 2.340 \\
15 & 0.222 & 0.026 & 2.506 & 47 & 0.226 & 0.025 & 2.480 \\
16 & 0.222 & 0.030 & 1.949 & 48 & 0.232 & 0.027 & 1.804 \\
17 & 0.226 & 0.026 & 2.614 & 49 & 0.223 & 0.029 & 1.981 \\
18 & 0.215 & 0.025 & 2.765 & 50 & 0.226 & 0.029 & 2.196 \\
19 & 0.217 & 0.026 & 2.798 & 51 & 0.231 & 0.033 & 1.369 \\
20 & 0.218 & 0.025 & 2.328 & 52 & 0.210 & 0.027 & 2.090 \\
21 & 0.218 & 0.026 & 2.599 & 53 & 0.215 & 0.026 & 2.330 \\
22 & 0.221 & 0.026 & 2.317 & 54 & 0.209 & 0.025 & 2.164 \\
23 & 0.215 & 0.025 & 2.520 & 55 & 0.222 & 0.025 & 2.717 \\
24 & 0.240 & 0.031 & 1.508 & 56 & 0.230 & 0.027 & 2.131 \\
25 & 0.220 & 0.025 & 2.814 & 57 & -- & -- &1.350 \\
26 & 0.213 & 0.025 & 2.948 & 58 & -- & -- &1.145 \\
27 & 0.228 & 0.026 & 2.740 & 59 & -- & -- &1.162 \\
28 & 0.228 & 0.029 & 2.157 & 60 & 0.250 & 0.034 & 1.438 \\
29 & 0.222 & 0.026 & 2.422 & 61 & 0.242 & 0.028 & 2.022 \\
30 & 0.227 & 0.025 & 2.896 & 62 & 0.257 & 0.030 & 1.743 \\
31 & 0.227 & 0.026 & 2.721 & 63 & 0.234 & 0.026 & 2.161 \\
32 & 0.235 & 0.027 & 1.987 & 64 & 0.238 & 0.029 & 1.916 \\
\bottomrule
\end{tabulary}
\caption[EC107--PMTB Efficiency Results]{ \label{tab:EC107--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC107_PMTC_AbsoluteMap_RefPixel038 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC107--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.129 & 33 & 0.267 & 0.030 & 1.837 \\
02 & -- & -- &1.542 & 34 & 0.239 & 0.025 & 2.951 \\
03 & 0.305 & 0.035 & 1.582 & 35 & 0.234 & 0.025 & 2.659 \\
04 & -- & -- &1.495 & 36 & 0.243 & 0.026 & 2.899 \\
05 & -- & -- &1.528 & 37 & 0.239 & 0.025 & 2.577 \\
06 & -- & -- &0.519 & 38 & 0.239 & 0.021 & 2.818 \\
07 & 0.287 & 0.031 & 1.627 & 39 & 0.239 & 0.025 & 2.429 \\
08 & 0.269 & 0.030 & 1.731 & 40 & 0.259 & 0.026 & 2.511 \\
09 & 0.271 & 0.035 & 1.418 & 41 & 0.240 & 0.025 & 2.728 \\
10 & 0.246 & 0.027 & 2.510 & 42 & 0.240 & 0.025 & 2.868 \\
11 & 0.236 & 0.026 & 2.542 & 43 & 0.233 & 0.025 & 3.010 \\
12 & 0.234 & 0.025 & 2.479 & 44 & 0.233 & 0.025 & 2.735 \\
13 & 0.245 & 0.028 & 2.092 & 45 & 0.236 & 0.025 & 2.405 \\
14 & 0.246 & 0.026 & 2.425 & 46 & 0.239 & 0.025 & 2.726 \\
15 & 0.255 & 0.027 & 2.273 & 47 & 0.243 & 0.026 & 3.384 \\
16 & 0.248 & 0.026 & 2.000 & 48 & 0.254 & 0.026 & 2.586 \\
17 & 0.260 & 0.026 & 2.661 & 49 & 0.245 & 0.025 & 2.853 \\
18 & 0.238 & 0.025 & 2.587 & 50 & 0.239 & 0.025 & 3.215 \\
19 & 0.241 & 0.026 & 2.676 & 51 & 0.236 & 0.025 & 2.840 \\
20 & 0.257 & 0.033 & 1.545 & 52 & 0.239 & 0.025 & 2.838 \\
21 & 0.245 & 0.027 & 2.406 & 53 & 0.243 & 0.030 & 1.945 \\
22 & 0.241 & 0.025 & 2.616 & 54 & 0.238 & 0.025 & 3.327 \\
23 & 0.240 & 0.025 & 2.626 & 55 & 0.245 & 0.025 & 2.922 \\
24 & 0.245 & 0.026 & 2.389 & 56 & 0.233 & 0.025 & 2.677 \\
25 & 0.247 & 0.025 & 2.494 & 57 & 0.275 & 0.030 & 1.924 \\
26 & 0.237 & 0.025 & 2.890 & 58 & 0.265 & 0.025 & 2.997 \\
27 & 0.238 & 0.026 & 2.788 & 59 & 0.270 & 0.025 & 2.824 \\
28 & 0.236 & 0.025 & 2.595 & 60 & 0.253 & 0.025 & 3.076 \\
29 & 0.237 & 0.025 & 2.472 & 61 & 0.260 & 0.024 & 2.729 \\
30 & 0.238 & 0.026 & 2.788 & 62 & 0.271 & 0.025 & 3.034 \\
31 & 0.247 & 0.026 & 2.664 & 63 & 0.269 & 0.025 & 2.687 \\
32 & 0.245 & 0.025 & 2.010 & 64 & 0.227 & 0.025 & 2.123 \\
\bottomrule
\end{tabulary}
\caption[EC107--PMTC Efficiency Results]{ \label{tab:EC107--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC107_PMTD_AbsoluteMap_RefPixel022 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC107--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.264 & 0.026 & 2.543 & 33 & 0.249 & 0.026 & 2.648 \\
02 & 0.250 & 0.026 & 2.393 & 34 & 0.231 & 0.025 & 2.832 \\
03 & 0.252 & 0.028 & 1.866 & 35 & 0.225 & 0.025 & 2.644 \\
04 & -- & -- &1.420 & 36 & 0.234 & 0.026 & 2.312 \\
05 & 0.243 & 0.026 & 2.163 & 37 & 0.244 & 0.035 & 1.643 \\
06 & 0.262 & 0.028 & 1.915 & 38 & 0.231 & 0.025 & 2.759 \\
07 & 0.256 & 0.027 & 2.005 & 39 & 0.242 & 0.027 & 2.095 \\
08 & 0.237 & 0.029 & 1.631 & 40 & 0.260 & 0.027 & 2.100 \\
09 & 0.237 & 0.025 & 2.984 & 41 & 0.244 & 0.025 & 2.900 \\
10 & 0.221 & 0.025 & 3.125 & 42 & 0.239 & 0.026 & 2.546 \\
11 & 0.217 & 0.025 & 3.137 & 43 & 0.226 & 0.025 & 3.055 \\
12 & 0.217 & 0.025 & 2.961 & 44 & 0.233 & 0.026 & 2.947 \\
13 & 0.219 & 0.025 & 3.029 & 45 & 0.234 & 0.026 & 3.118 \\
14 & 0.227 & 0.025 & 2.760 & 46 & 0.229 & 0.026 & 2.983 \\
15 & 0.233 & 0.025 & 3.008 & 47 & 0.240 & 0.026 & 2.704 \\
16 & 0.235 & 0.026 & 2.094 & 48 & 0.268 & 0.028 & 2.163 \\
17 & 0.243 & 0.025 & 3.004 & 49 & 0.262 & 0.029 & 2.176 \\
18 & 0.223 & 0.026 & 2.920 & 50 & 0.240 & 0.026 & 2.176 \\
19 & 0.217 & 0.025 & 2.827 & 51 & 0.261 & 0.033 & 1.614 \\
20 & 0.222 & 0.026 & 2.820 & 52 & 0.237 & 0.027 & 2.185 \\
21 & 0.225 & 0.026 & 2.648 & 53 & 0.238 & 0.026 & 2.585 \\
22 & 0.223 & 0.021 & 2.616 & 54 & 0.249 & 0.026 & 2.502 \\
23 & 0.236 & 0.026 & 2.593 & 55 & 0.246 & 0.026 & 2.176 \\
24 & 0.254 & 0.032 & 1.747 & 56 & 0.264 & 0.027 & 2.381 \\
25 & 0.249 & 0.025 & 2.564 & 57 & 0.296 & 0.035 & 1.395 \\
26 & 0.228 & 0.025 & 3.222 & 58 & -- & -- &1.116 \\
27 & 0.216 & 0.025 & 2.765 & 59 & -- & -- &1.316 \\
28 & 0.212 & 0.025 & 2.205 & 60 & 0.290 & 0.034 & 1.470 \\
29 & 0.218 & 0.026 & 2.521 & 61 & 0.285 & 0.029 & 1.736 \\
30 & 0.227 & 0.026 & 2.612 & 62 & 0.289 & 0.028 & 1.730 \\
31 & 0.235 & 0.026 & 2.900 & 63 & 0.283 & 0.028 & 1.939 \\
32 & 0.248 & 0.026 & 2.203 & 64 & -- & -- &1.172 \\
\bottomrule
\end{tabulary}
\caption[EC107--PMTD Efficiency Results]{ \label{tab:EC107--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC108_PMTA_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC108--PMTA}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.373 & 33 & 0.268 & 0.032 & 1.349 \\
02 & 0.245 & 0.029 & 1.710 & 34 & 0.214 & 0.027 & 1.860 \\
03 & 0.246 & 0.028 & 1.572 & 35 & -- & -- &1.670 \\
04 & 0.252 & 0.028 & 1.927 & 36 & 0.221 & 0.027 & 2.205 \\
05 & 0.258 & 0.030 & 1.616 & 37 & 0.223 & 0.027 & 2.222 \\
06 & 0.267 & 0.029 & 1.799 & 38 & 0.217 & 0.025 & 2.501 \\
07 & 0.281 & 0.031 & 1.956 & 39 & 0.230 & 0.027 & 2.364 \\
08 & 0.275 & 0.033 & 1.489 & 40 & 0.233 & 0.028 & 1.749 \\
09 & 0.242 & 0.027 & 2.048 & 41 & 0.244 & 0.031 & 1.519 \\
10 & 0.214 & 0.025 & 2.879 & 42 & -- & -- &1.383 \\
11 & 0.218 & 0.025 & 2.762 & 43 & -- & -- &0.661 \\
12 & 0.212 & 0.025 & 2.928 & 44 & 0.216 & 0.027 & 2.170 \\
13 & 0.225 & 0.027 & 2.482 & 45 & 0.233 & 0.034 & 1.614 \\
14 & 0.224 & 0.025 & 2.838 & 46 & -- & -- &0.370 \\
15 & -- & -- &1.339 & 47 & 0.223 & 0.025 & 2.548 \\
16 & 0.253 & 0.029 & 2.035 & 48 & 0.238 & 0.031 & 1.758 \\
17 & 0.236 & 0.021 & 3.104 & 49 & -- & -- &0.903 \\
18 & 0.219 & 0.026 & 2.536 & 50 & -- & -- &1.404 \\
19 & 0.208 & 0.025 & 2.790 & 51 & -- & -- &1.467 \\
20 & -- & -- &1.051 & 52 & 0.224 & 0.027 & 2.140 \\
21 & 0.215 & 0.026 & 2.561 & 53 & -- & -- &1.143 \\
22 & 0.219 & 0.027 & 2.306 & 54 & 0.213 & 0.025 & 2.796 \\
23 & 0.242 & 0.032 & 1.903 & 55 & 0.222 & 0.026 & 2.621 \\
24 & 0.247 & 0.027 & 2.031 & 56 & 0.218 & 0.029 & 1.449 \\
25 & 0.244 & 0.026 & 2.219 & 57 & -- & -- &0.319 \\
26 & 0.221 & 0.027 & 2.486 & 58 & -- & -- &0.624 \\
27 & 0.209 & 0.025 & 2.338 & 59 & -- & -- &0.541 \\
28 & 0.236 & 0.031 & 1.777 & 60 & -- & -- &0.911 \\
29 & 0.216 & 0.027 & 2.453 & 61 & 0.251 & 0.033 & 1.565 \\
30 & 0.220 & 0.025 & 2.743 & 62 & -- & -- &1.096 \\
31 & -- & -- &0.688 & 63 & -- & -- &1.158 \\
32 & 0.238 & 0.029 & 1.736 & 64 & -- & -- &0.387 \\
\bottomrule
\end{tabulary}
\caption[EC108--PMTA Efficiency Results]{ \label{tab:EC108--PMTA EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC108_PMTB_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC108--PMTB}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.200 & 0.027 & 2.123 & 33 & 0.215 & 0.028 & 2.165 \\
02 & 0.206 & 0.026 & 2.257 & 34 & 0.209 & 0.033 & 1.482 \\
03 & 0.220 & 0.026 & 2.604 & 35 & 0.204 & 0.028 & 1.818 \\
04 & -- & -- &0.703 & 36 & 0.194 & 0.026 & 2.043 \\
05 & 0.239 & 0.034 & 1.580 & 37 & -- & -- &1.065 \\
06 & 0.230 & 0.035 & 1.407 & 38 & 0.208 & 0.029 & 2.226 \\
07 & -- & -- &1.195 & 39 & 0.201 & 0.027 & 2.366 \\
08 & -- & -- &0.667 & 40 & 0.192 & 0.027 & 1.958 \\
09 & 0.204 & 0.026 & 2.434 & 41 & 0.204 & 0.026 & 2.385 \\
10 & 0.205 & 0.026 & 2.800 & 42 & -- & -- &0.687 \\
11 & 0.202 & 0.026 & 2.825 & 43 & 0.206 & 0.027 & 2.063 \\
12 & 0.204 & 0.026 & 2.551 & 44 & 0.222 & 0.034 & 1.683 \\
13 & 0.197 & 0.026 & 1.818 & 45 & 0.201 & 0.027 & 2.009 \\
14 & -- & -- &1.470 & 46 & 0.201 & 0.026 & 2.383 \\
15 & -- & -- &1.000 & 47 & 0.208 & 0.026 & 2.035 \\
16 & -- & -- &1.079 & 48 & 0.200 & 0.033 & 1.669 \\
17 & 0.213 & 0.021 & 3.058 & 49 & 0.208 & 0.028 & 1.854 \\
18 & 0.210 & 0.027 & 2.276 & 50 & 0.211 & 0.031 & 2.005 \\
19 & 0.204 & 0.027 & 2.473 & 51 & 0.213 & 0.032 & 1.639 \\
20 & 0.208 & 0.028 & 2.373 & 52 & 0.205 & 0.030 & 1.741 \\
21 & 0.204 & 0.027 & 2.236 & 53 & 0.197 & 0.027 & 2.063 \\
22 & 0.214 & 0.034 & 1.797 & 54 & 0.208 & 0.028 & 2.035 \\
23 & 0.205 & 0.027 & 1.793 & 55 & 0.196 & 0.025 & 2.491 \\
24 & -- & -- &1.354 & 56 & 0.182 & 0.027 & 1.940 \\
25 & 0.204 & 0.025 & 2.563 & 57 & 0.219 & 0.033 & 1.523 \\
26 & 0.208 & 0.026 & 2.498 & 58 & -- & -- &0.642 \\
27 & -- & -- &0.410 & 59 & -- & -- &1.304 \\
28 & -- & -- &1.214 & 60 & -- & -- &1.258 \\
29 & 0.201 & 0.028 & 2.321 & 61 & 0.225 & 0.030 & 1.662 \\
30 & -- & -- &0.355 & 62 & 0.230 & 0.029 & 1.876 \\
31 & 0.213 & 0.033 & 1.627 & 63 & 0.213 & 0.029 & 1.668 \\
32 & 0.203 & 0.033 & 1.475 & 64 & 0.180 & 0.033 & 1.379 \\
\bottomrule
\end{tabulary}
\caption[EC108--PMTB Efficiency Results]{ \label{tab:EC108--PMTB EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC108_PMTC_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC108--PMTC}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & -- & -- &1.542 & 33 & 0.195 & 0.028 & 1.682 \\
02 & 0.182 & 0.026 & 1.925 & 34 & 0.179 & 0.027 & 2.295 \\
03 & 0.203 & 0.027 & 1.819 & 35 & 0.182 & 0.029 & 2.026 \\
04 & 0.201 & 0.028 & 1.701 & 36 & 0.177 & 0.025 & 3.850 \\
05 & -- & -- &1.314 & 37 & 0.183 & 0.025 & 2.823 \\
06 & -- & -- &1.288 & 38 & 0.179 & 0.025 & 3.444 \\
07 & -- & -- &1.507 & 39 & 0.195 & 0.025 & 3.174 \\
08 & -- & -- &1.067 & 40 & 0.172 & 0.027 & 2.260 \\
09 & 0.192 & 0.026 & 2.256 & 41 & 0.205 & 0.028 & 1.869 \\
10 & 0.172 & 0.025 & 3.500 & 42 & 0.195 & 0.032 & 2.119 \\
11 & 0.186 & 0.026 & 3.008 & 43 & -- & -- &0.658 \\
12 & 0.184 & 0.026 & 2.734 & 44 & 0.178 & 0.026 & 3.252 \\
13 & 0.191 & 0.026 & 2.438 & 45 & 0.174 & 0.026 & 2.636 \\
14 & 0.185 & 0.026 & 2.656 & 46 & -- & -- &0.393 \\
15 & 0.195 & 0.031 & 1.548 & 47 & 0.187 & 0.026 & 3.315 \\
16 & 0.167 & 0.029 & 1.695 & 48 & 0.161 & 0.026 & 2.532 \\
17 & 0.186 & 0.022 & 2.437 & 49 & -- & -- &1.345 \\
18 & 0.176 & 0.025 & 3.172 & 50 & 0.204 & 0.034 & 1.871 \\
19 & 0.176 & 0.026 & 2.805 & 51 & 0.198 & 0.030 & 1.940 \\
20 & 0.203 & 0.035 & 1.771 & 52 & 0.190 & 0.025 & 2.945 \\
21 & 0.181 & 0.026 & 3.235 & 53 & 0.202 & 0.034 & 1.315 \\
22 & 0.194 & 0.027 & 2.521 & 54 & 0.191 & 0.025 & 3.787 \\
23 & 0.194 & 0.027 & 2.331 & 55 & 0.185 & 0.026 & 3.533 \\
24 & 0.172 & 0.026 & 2.064 & 56 & 0.164 & 0.027 & 2.211 \\
25 & 0.190 & 0.026 & 2.759 & 57 & -- & -- &0.784 \\
26 & 0.179 & 0.025 & 3.195 & 58 & -- & -- &0.890 \\
27 & 0.175 & 0.025 & 3.398 & 59 & -- & -- &1.312 \\
28 & 0.179 & 0.026 & 3.085 & 60 & 0.205 & 0.029 & 1.768 \\
29 & 0.183 & 0.025 & 3.349 & 61 & 0.203 & 0.025 & 2.916 \\
30 & 0.188 & 0.026 & 2.900 & 62 & 0.193 & 0.025 & 3.056 \\
31 & -- & -- &0.719 & 63 & 0.198 & 0.027 & 2.679 \\
32 & 0.172 & 0.026 & 2.183 & 64 & 0.179 & 0.032 & 1.864 \\
\bottomrule
\end{tabulary}
\caption[EC108--PMTC Efficiency Results]{ \label{tab:EC108--PMTC EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC108_PMTD_AbsoluteMap_RefPixel017 <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC || LCCC}
\multicolumn{4}{l}{EC108--PMTD}\\
\toprule
Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V & Pixel & $\epsilon$ & $\delta \epsilon/\epsilon$ & P/V \\
\cmidrule(l){1-8}
01 & 0.279 & 0.029 & 2.020 & 33 & 0.254 & 0.025 & 2.487 \\
02 & 0.259 & 0.025 & 2.608 & 34 & 0.264 & 0.030 & 1.967 \\
03 & 0.241 & 0.025 & 2.584 & 35 & 0.242 & 0.026 & 2.392 \\
04 & -- & -- &0.819 & 36 & 0.247 & 0.027 & 2.627 \\
05 & 0.250 & 0.027 & 2.020 & 37 & -- & -- &1.252 \\
06 & 0.281 & 0.036 & 1.445 & 38 & 0.241 & 0.025 & 2.860 \\
07 & -- & -- &1.240 & 39 & 0.250 & 0.026 & 2.721 \\
08 & -- & -- &0.790 & 40 & 0.256 & 0.026 & 2.391 \\
09 & 0.256 & 0.025 & 3.004 & 41 & 0.253 & 0.025 & 2.603 \\
10 & 0.254 & 0.025 & 3.249 & 42 & -- & -- &0.573 \\
11 & 0.253 & 0.025 & 3.527 & 43 & 0.240 & 0.025 & 2.617 \\
12 & 0.244 & 0.025 & 3.279 & 44 & 0.251 & 0.026 & 2.600 \\
13 & 0.244 & 0.026 & 2.108 & 45 & 0.244 & 0.027 & 2.204 \\
14 & 0.250 & 0.030 & 1.980 & 46 & 0.243 & 0.025 & 2.767 \\
15 & -- & -- &1.212 & 47 & 0.253 & 0.025 & 2.642 \\
16 & -- & -- &1.101 & 48 & 0.270 & 0.028 & 1.986 \\
17 & 0.259 & 0.021 & 0.005 & 49 & 0.256 & 0.026 & 2.142 \\
18 & 0.240 & 0.025 & 2.708 & 50 & 0.258 & 0.028 & 1.996 \\
19 & 0.240 & 0.025 & 3.121 & 51 & 0.250 & 0.027 & 2.024 \\
20 & 0.241 & 0.025 & 2.727 & 52 & -- & -- &1.629 \\
21 & 0.234 & 0.025 & 3.136 & 53 & 0.254 & 0.026 & 2.828 \\
22 & 0.234 & 0.027 & 2.361 & 54 & 0.249 & 0.025 & 2.541 \\
23 & 0.252 & 0.026 & 2.232 & 55 & 0.253 & 0.025 & 2.723 \\
24 & -- & -- &1.479 & 56 & 0.273 & 0.028 & 2.262 \\
25 & 0.238 & 0.025 & 3.016 & 57 & 0.306 & 0.035 & 1.312 \\
26 & 0.245 & 0.025 & 2.910 & 58 & -- & -- &0.436 \\
27 & -- & -- &0.453 & 59 & 0.289 & 0.034 & 1.506 \\
28 & 0.240 & 0.026 & 2.255 & 60 & 0.304 & 0.035 & 1.453 \\
29 & 0.240 & 0.025 & 2.727 & 61 & 0.274 & 0.027 & 1.764 \\
30 & -- & -- &0.751 & 62 & 0.285 & 0.030 & 1.696 \\
31 & 0.239 & 0.026 & 2.548 & 63 & 0.284 & 0.027 & 1.831 \\
32 & 0.256 & 0.027 & 1.726 & 64 & -- & -- &1.114 \\
\bottomrule
\end{tabulary}
\caption[EC108--PMTD Efficiency Results]{ \label{tab:EC108--PMTD EffResults}}
\end{center}
\end{table}


==> tables/EUSOBalloon-ECmeasurements/LatexTable_EC109_PMTD_GainMap <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC||LCCC}
\multicolumn{4}{l}{EC109--PMTD}\\
\toprule
Pixel & $\mu$ & $\delta \mu/\mu$ & P/V & Pixel & $\mu$ & $\delta \mu/\mu$ & P/V\\
\cmidrule(l){1-8}
01 & 5.46 & 0.01 & 1.87 & 33 & 6.68 & 0.01 & 2.50 \\
02 & 5.84 & 0.01 & 2.61 & 34 & 7.06 & 0.01 & 2.30 \\
03 & 6.16 & 0.01 & 2.73 & 35 & 6.47 & 0.01 & 3.27 \\
04 & 6.54 & 0.01 & 2.20 & 36 & 6.55 & 0.01 & 3.20 \\
05 & 5.93 & 0.01 & 2.58 & 37 & 6.59 & 0.01 & 2.17 \\
06 & 6.15 & 0.01 & 1.48 & 38 & 6.70 & 0.01 & 3.06 \\
07 & 6.26 & 0.01 & 1.80 & 39 & 6.95 & 0.01 & 3.11 \\
08 & 11.86 & 0.02 & 0.79 & 40 & 7.34 & 0.01 & 2.54 \\
09 & 7.28 & 0.01 & 3.27 & 41 & 6.39 & 0.01 & 2.94 \\
10 & 7.86 & 0.01 & 3.68 & 42 & 6.17 & 0.01 & 3.19 \\
11 & 7.60 & 0.01 & 3.56 & 43 & 6.15 & 0.01 & 3.45 \\
12 & 7.52 & 0.01 & 3.64 & 44 & 6.41 & 0.01 & 2.79 \\
13 & 7.61 & 0.01 & 3.33 & 45 & 6.14 & 0.01 & 3.18 \\
14 & 7.71 & 0.01 & 2.94 & 46 & 6.56 & 0.01 & 3.49 \\
15 & 7.87 & 0.01 & 1.89 & 47 & 7.04 & 0.01 & 3.27 \\
16 & 7.53 & 0.01 & 1.20 & 48 & 7.14 & 0.01 & 2.45 \\
17 & 7.23 & 0.01 & 3.12 & 49 & 6.53 & 0.01 & 2.16 \\
18 & 7.44 & 0.01 & 3.83 & 50 & 6.30 & 0.01 & 2.95 \\
19 & 7.16 & 0.01 & 4.17 & 51 & 6.40 & 0.01 & 1.96 \\
20 & 7.31 & 0.01 & 3.51 & 52 & 6.56 & 0.01 & 3.34 \\
21 & 7.17 & 0.01 & 3.50 & 53 & 6.29 & 0.01 & 3.07 \\
22 & 7.27 & 0.01 & 3.30 & 54 & 6.28 & 0.01 & 3.15 \\
23 & 7.56 & 0.01 & 2.98 & 55 & 6.93 & 0.01 & 3.20 \\
24 & 7.71 & 0.01 & 1.34 & 56 & 6.68 & 0.01 & 2.34 \\
25 & 7.15 & 0.01 & 2.95 & 57 & 4.72 & 0.01 & 0.83 \\
26 & 7.22 & 0.01 & 2.84 & 58 & 4.78 & 0.01 & 1.02 \\
27 & 6.96 & 0.01 & 3.27 & 59 & 4.79 & 0.01 & 1.53 \\
28 & 6.97 & 0.01 & 2.37 & 60 & 5.23 & 0.01 & 1.82 \\
29 & 6.67 & 0.01 & 2.92 & 61 & 5.16 & 0.01 & 2.09 \\
30 & 6.38 & 0.01 & 2.67 & 62 & 4.94 & 0.01 & 1.85 \\
31 & 6.86 & 0.01 & 3.06 & 63 & 5.29 & 0.01 & 2.31 \\
32 & 7.46 & 0.01 & 2.53 & 64 & 2.88 & 0.04 & 0.00 \\
\bottomrule
\end{tabulary}
\caption[EC109--PMTD Gain Results]{ \label{tab:EC109--PMTD gainResults}}
\end{center}
\end{table}


==> tables/HamamatsuLowCurrentVoltageDis.tex <==
\begin{table}
 \begin{center}
\begin{tabular}{l|c|r}
PMT Element & Ratio& Voltages [V] \\ \hline		
$K$ & $2.9$&	$1000$ \\
$D1$&	$1$& $805$	\\
$D2$& $1$& 	$738$	\\
$D3$& $1$& 	$671$	\\
$D4$& $1$& 	$604$ 	\\
$D5$& $1$& 	$537$ 	\\
$D6$& $1$& 	$470$\\
$D7$& $1$& 	$403$	\\
$D8$& $1$& 	$336$ \\
$D9$& $1$& $268$ 	\\
$D10$& $1$& 	$201$	\\
$D11$& $1$& 	$134$ 	\\
$D12$& $0.67$& 	$67$ 	\\
$G$& $0.33$& 	$22$ 	\\
\end{tabular}
\caption[Low Power Voltage Distribution]{The modified voltage distribution for the M64 PMT designed to reduce the overall power consumption 
of the tube and to simplify the design of the Cockcroft–Walton power-supply.}
\label{tab:HamamatsuLowCurrentVoltageDis}
\end{center}
\end{table}


==> tables/HamamatsuResistiveVoltageDis.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{l|c|c|l}
PMT Element & Ratio & Voltages [V] & Scaled-Up Voltages [V] \\ \hline	
$K$ & $2.3$&	$1000$& $1100$\\
$D1$& $1.2$&	$847$&	$931$\\
$D2$& $1$&	$767$&	$843$\\
$D3$& $1$&	$700$&	$770$\\
$D4$& $1$&	$633$ & $697$\\
$D5$& $1$&	$567$ &	$623$\\
$D6$& $1$&	$500$& 	$550$\\
$D7$& $1$&	$433$& 	$477$\\
$D8$& $1$&	$367$ &	$403$\\
$D9$& $1$&	$300$ & $330$\\
$D10$& $1$&	$233$&	$257$\\
$D11$& $1$&	$167$ & $183$\\
$D12$& $1$&	$100$ &	$110$\\
$G$& $0.5$&	$33$ &	$37$\\
\end{tabular}
\caption[Hamamatsu Voltage Distribution]{``Normal'' voltage distribution as specified by Hamamatsu for the M64 PMT.}
\label{tab:HamamatsuResistiveVoltageDis}
\end{center}
\end{table}


==> tables/IntroToJEMEUSO/JEMEUSOspecifications_short.tex <==

\begin{table}
 \begin{center}
\begin{tabulary}{1.0\textwidth}{LLL}
\toprule
Parameter & Value & Note(s)\\
\cmidrule(l){1-3}
\alert{\emph{Optics}} & & \\ 
% \cmidrule(l){1-2}
Optical Aperture & 4.5 m$^{2}$ & Baseline\\
% Ensquared Collection Efficiency & 35\% (15\%) & For $\lambda = 350~$nm\\
% Ensquared Energy & 86\% (80\%) & For $\lambda = 350~$nm\\
Optical Bandwidth & 290-430 nm & \\
% Field of View & 0.85 sr & \\
Observational Area & $1.4~10^{5}~$km$^{2}$\\
 & & \\
\alert{\emph{FS Detector and Electronics}} & &  \\ 
% \cmidrule(l){1-2}
Number of Pixels & $3.2~10^{5}$ & \\
Spatial Angular Resolution & $0.074^{\circ}$ & \\
Pixel Size at Ground & 0.51 km & For $H_{o}=400~$km\\
PMT efficiency & $\sim32 \%$ & For $\lambda = 350~$nm \\
Cross Talk & $< 2\%$ & \\
Transmittance of UV filter (BG3) & 97\% & For $\lambda = 350~$nm \\
Sampling Time & $2.5~\mu$s & ``TPC''\\
\end{tabulary}
\caption[JEM-EUSO Characteristics]{
\label{tab:JEMEUSOCharacteristics}
% The characteristics of the JEM-EUSO telescope design. Values apply at the center of the FoV, while values in parenthesis apply at the edge of the FoV.
% The ensquared collection efficiency is the ratio of the number of photons focused within a pixel area to the number incident on the entrance aperture of the optics.
% Similarly, the ensquared energy is ratio of photons focused within the area of a pixel to those reaching the focal surface.
}
 \end{center}
\end{table}



==> tables/PhototubeSorting/LatexTable_EC109_PMTD_GainMap <==
\begin{table}
\begin{center}
\begin{tabulary}{1.0\textwidth}{LCCC||LCCC}
\multicolumn{4}{l}{EC109--PMTD}\\
\toprule
Pixel & $\mu$ & $\delta \mu/\mu$ & P/V & Pixel & $\mu$ & $\delta \mu/\mu$ & P/V\\
\cmidrule(l){1-8}
01 & 5.46 & 0.01 & 1.87 & 33 & 6.68 & 0.01 & 2.50 \\
02 & 5.84 & 0.01 & 2.61 & 34 & 7.06 & 0.01 & 2.30 \\
03 & 6.16 & 0.01 & 2.73 & 35 & 6.47 & 0.01 & 3.27 \\
04 & 6.54 & 0.01 & 2.20 & 36 & 6.55 & 0.01 & 3.20 \\
05 & 5.93 & 0.01 & 2.58 & 37 & 6.59 & 0.01 & 2.17 \\
06 & 6.15 & 0.01 & 1.48 & 38 & 6.70 & 0.01 & 3.06 \\
07 & 6.26 & 0.01 & 1.80 & 39 & 6.95 & 0.01 & 3.11 \\
08 & 11.86 & 0.02 & 0.79 & 40 & 7.34 & 0.01 & 2.54 \\
09 & 7.28 & 0.01 & 3.27 & 41 & 6.39 & 0.01 & 2.94 \\
10 & 7.86 & 0.01 & 3.68 & 42 & 6.17 & 0.01 & 3.19 \\
11 & 7.60 & 0.01 & 3.56 & 43 & 6.15 & 0.01 & 3.45 \\
12 & 7.52 & 0.01 & 3.64 & 44 & 6.41 & 0.01 & 2.79 \\
13 & 7.61 & 0.01 & 3.33 & 45 & 6.14 & 0.01 & 3.18 \\
14 & 7.71 & 0.01 & 2.94 & 46 & 6.56 & 0.01 & 3.49 \\
15 & 7.87 & 0.01 & 1.89 & 47 & 7.04 & 0.01 & 3.27 \\
16 & 7.53 & 0.01 & 1.20 & 48 & 7.14 & 0.01 & 2.45 \\
17 & 7.23 & 0.01 & 3.12 & 49 & 6.53 & 0.01 & 2.16 \\
18 & 7.44 & 0.01 & 3.83 & 50 & 6.30 & 0.01 & 2.95 \\
19 & 7.16 & 0.01 & 4.17 & 51 & 6.40 & 0.01 & 1.96 \\
20 & 7.31 & 0.01 & 3.51 & 52 & 6.56 & 0.01 & 3.34 \\
21 & 7.17 & 0.01 & 3.50 & 53 & 6.29 & 0.01 & 3.07 \\
22 & 7.27 & 0.01 & 3.30 & 54 & 6.28 & 0.01 & 3.15 \\
23 & 7.56 & 0.01 & 2.98 & 55 & 6.93 & 0.01 & 3.20 \\
24 & 7.71 & 0.01 & 1.34 & 56 & 6.68 & 0.01 & 2.34 \\
25 & 7.15 & 0.01 & 2.95 & 57 & 4.72 & 0.01 & 0.83 \\
26 & 7.22 & 0.01 & 2.84 & 58 & 4.78 & 0.01 & 1.02 \\
27 & 6.96 & 0.01 & 3.27 & 59 & 4.79 & 0.01 & 1.53 \\
28 & 6.97 & 0.01 & 2.37 & 60 & 5.23 & 0.01 & 1.82 \\
29 & 6.67 & 0.01 & 2.92 & 61 & 5.16 & 0.01 & 2.09 \\
30 & 6.38 & 0.01 & 2.67 & 62 & 4.94 & 0.01 & 1.85 \\
31 & 6.86 & 0.01 & 3.06 & 63 & 5.29 & 0.01 & 2.31 \\
32 & 7.46 & 0.01 & 2.53 & 64 & 2.88 & 0.04 & 0.00 \\
\bottomrule
\end{tabulary}
\caption[EC109--PMTD Gain Results]{ \label{tab:EC109--PMTD gainResults}}
\end{center}
\end{table}

